Bandwidth-Aware Page Placement in NUMA

Page placement is a critical problem for memoryintensive applications running on a shared-memory multiprocessor with a non-uniform memory access (NUMA) architecture. State-of-the-art page placement mechanisms interleave pages evenly across NUMA nodes. However, this approach fails to maximize memory throughput in modern NUMA systems, characterised by asymmetric bandwidths and latencies, and sensitive to memory contention and interconnect congestion phenomena. We propose BWAP, a novel page placement mechanism based on asymmetric weighted page interleaving. BWAP combines an analytical performance model of the target NUMA system with on-line iterative tuning of page distribution for a given memory-intensive application. Our experimental evaluation with representative memory-intensive workloads shows that BWAP performs up to 66% better than state-of-the-art techniques. These gains are particularly relevant when multiple co-located applications run in disjoint partitions of a large NUMA machine or when applications do not scale up to the total number of cores.

==> background.tex <==

%%%%%%%%%%%   BACKGROUND   %%%%%%%%%%%
\section{Background}
\label{bg}

In this section, we provide some background on blockchains in general and Ethereum in particular.
We focus on the general high-level aspects rather than the low-level protocol details and formats.
For the latter, the interested reader can refer to the Ethereum's yellow paper~\cite{Ethereum} and the official Ethereum documentation~\cite{etherdocs}.
%In this section we give a brief introduction to Ethereum, adding the details that will be needed later in this paper.
Ethereum is a permissionless blockchain that provides a platform for developing and implementing decentralized applications --- known as Smart Contracts.
Ethereum also acts as a cryptocurrency by providing its own currency, known as Ether. 
Both the state of the currency and of the Smart Contracts is maintained in the blockchain, a public append-only ledger that keeps track of all state changes. 
The state of the system is associated with accounts, which are stateful objects whose states --- e.g. account balance or Smart Contract variable --- can be changed through transactions.
There are two types of accounts: externally owned ones which are controlled by user's private keys and contract accounts associated to Smart Contract code. %represented by a code controlled by messages.

The system runs on a peer-to-peer network basically consisting of three types of peers:
\begin{description}
  \item [Bootstrap nodes:] Highly-available peers run by volunteers whose purpose is to facilitate the connection of new clients.
  \item [Miners:] Peers who produce --- i.e. \emph{mine} ---  new blocks and spread them across the network.
  \item [End users:] Common participants of the platform that send and receive transactions, deploy smart contracts, etc.
\end{description}


In the rest of the section, we provide an overview of the main concepts underlying Ethereum.


\subsection{Transactions}
Transactions are the main mechanism to update the state of the system.
All transactions are signed by the account that submitted them to the system.
%refers to the signed data package assembled by externally owned accounts.
Transactions have two different uses: i) to indicate a simple currency transfer between accounts or, ii) to deploy or invoke operations in Smart Contracts.
%They are later propagated to the network as described in Section~\ref{tx-lifecycle}. 	
A transaction contains several fields, of which the most important are: the address (public key) of the recipient, the value of Ether to be sent, the Smart Contract code, and the \emph{nonce} indicating the total number of transactions sent from the account, and used to ensure the transactions emitted from an account are executed in the desired order.

To prevent flooding the platform with useless or spurious transactions, as well as to forbid the execution of Smart Contracts with infinite loops, Ethereum implements an internal pricing system in the form of gas. 
Each transaction's code -- be it a simple value transfer or a contract call -- is a collection of opcodes, where each opcode costs a pre-determined amount of gas. 
The creator of the transaction cannot modify this cost, but she is free to choose the \emph{gas price} --- the amount of Ether she is willing to pay per one unit of gas to the miner for including such transaction in a block. The transaction fee then equates to the product of the amount of gas spent and gas price per unit.


\subsubsection{Transaction lifecycle}
\label{tx-lifecycle}

Transactions are disseminated over the network using an epidemic, or gossip-based, protocol.
Briefly, when a user creates a new transaction, she broadcasts it to all the neighboring peers.
Upon a transaction reception, the nodes forward the transaction to their neighbors -- usually just to a limited number of them -- which in turn will forward it to their neighbors.
Eventually, the transaction will reach a miner node.
Miners perform a process called \emph{mining} -- described in more detail in \S\ref{subsec:mining} -- which leads to the insertion of the transaction into a new block. 
Miners then propagate the block back to the network also following a gossip style protocol.
Peers eventually receive the block, verify its validity, and update accordingly their local copy of the blockchain.

It is important to note that the information propagation strategies and the client behavior in general are not standardized in Ethereum. 
For instance, the Geth client (v1.8.23) maintains connections with 25 other nodes, whereas Parity connects to 50 peers.
Currently, there are 8 different client implementations written in different languages, all following the WIRE\footnote{https://github.com/ethereum/devp2p/blob/master/caps/eth.md} protocol specification, but their logic substantially differs from each other.
This heterogeneity implies that it is challenging to accurately infer the behavior of the network by carefully studying all implementations, and rather one needs to resort to observing and measuring such behavior in the real deployment over a long time period.


\subsection{Blockchain forks}
The Ethereum protocol aims for a block interval -- the mean time it takes to mine a new block -- between ten to twenty seconds. 
This is ensured by continuously and automatically adjusting the mining difficulty.
On one hand, the low block interval -- $\sim$40 times shorter than in Bitcoin --  allows for better response time, which is a desired property in cryptocurrencies, and for better throughput.
 On the other hand, short block intervals lead to an increased amount of forks, i.e. events where two competing miners produce two blocks that reference the same preceding block.


%Huge forked block rates in classical Nakamoto's consensus impede less powerful miners, as they are less likely to mine a block fast enough, thus leading to mining centralization. They also weaken the absolute strength of the network against attacks, as the inventor and co-creator of Ethereum Vitalik Buterin explains in his blog post\footnote{https://blog.ethereum.org/2014/07/11/toward-a-12-second-block-time/}.
%Ethereum, as a countermeasure against the unpleasant consequences of the short block interval, implements a modified version of the Greedy Heaviest Observed Subtree (GHOST) protocol~\cite{GHOST}.
Given a fork, miners have to decide which path to consider as valid.
The original Nakamoto's consensus protocol~\cite{Bitcoin} considers the longest chain as the one which represents the current state of a blockchain network.
This implies that blocks that are not included in the main chain are discarded, together with the mining effort spent to produce such blocks.
Ethereum adopts another strategy by relying on a modified version of the Greedy Heaviest Observed Subtree (GHOST) protocol~\cite{GHOST}.
The intuition is simple, rather than completely discarding blocks that did not end up in the main chain, Ethereum allows blocks in the main chain to reference blocks outside the main chain --- known as uncle blocks.
Therefore, the weight of a chain is calculated from the cumulative difficulty of the main chain and uncles. 
The Ethereum GHOST modification deviates from the original one in the fact that it rewards not just the blocks on the main chain, but the uncles as well. 
The goal is to incentivize small miners, and hence mining decentralization, by promoting a fairer distribution of rewards among miners.
Moreover, this also strengthens the security of the blockchain as a malicious actor needs to construct a chain that is \emph{heavier} than the main chain plus the corresponding uncle blocks.
Finally, blocks that are not included in the main chain nor referenced by any blocks are called unrecognized forks and do not contribute to the security of the blockchain.


Note that despite the fact that Ethereum distributes rewards to uncle blocks, only transactions included in main blocks affect the state of the system and transactions in the uncle blocks are ignored.
When coupled with the occurrence of forks, this implies that when a node observes a new block B, it is not safe to immediately consider the state transition given by the transactions in block B, because there is a chance that B might be considered an uncle or unrecognized block at a later point in time.
Therefore, nodes must wait for a \emph{long enough} suffix of blocks to ensure that the appearance of an alternative heavier chain, where block B is not included, has a small probability. 
This property is known as block finality.
In Ethereum, nodes wait for a suffix of 12 blocks before considering a block final --- and thus consider the transactions that affect the blockchain state valid~\cite{blockConfirmation}.
Note, however, that due to the nature of Proof-of-Work (PoW), block finality is always probabilistic as there is always a non-zero chance that an alternative heavier chain appears.


Our observations, discussed in more detail in \S\ref{Analysis}, provide some surprising results on the topics we just discussed.
On the one hand, the rewards of uncle blocks, which are supposed to incentivize a fairer share of rewards, are in fact being exploited by mining pools to further increase their gains.
On the other hand, we observed that mining pools have been able to mine large continuous sequence of blocks putting into question the rule of thumb of the 12 confirmation blocks.


\subsection{Mining process}
\label{subsec:mining}
The role of miners is to validate transactions and orderly collect them in blocks.
Mining rewards a successful miner with a fixed amount of Ether coins per block, along with transaction fees for every transaction included in the newly mined block.

\subsubsection{Proof-of-work}
Miners, in addition to validating transactions, must perform a technique called Proof-of-Work (PoW) which consists of resolving a computationally expensive cryptopuzzles.
Under the hood, PoW consists of repetitive hashing of a string consisting of the block's data and a nonce.
The goal is to find a nonce such that the resulting hash is less than a certain threshold -- determined by the difficulty of the network. 
Because the hash function is assumed to be practically non-invertible, the only way to solve the puzzle is through brute force.
After finding a solution, the block is valid and can be propagated to the network.
%A miner tries to perform the computations for a tremendous number of nonces until the final produced hash 
% TODO     - more reasons for pOw -> ( preventing Sybil attacks ?? )
The fact that PoW is very hard to perform guarantees the security of the platform since it makes it resistant to being flooded by false blocks and makes potential future modifications of previously confirmed parts of the blockchain almost impossible. Furthermore, it makes miners spend some time performing the computations, allowing the rest of the network to have enough time to synchronize.
Due to the computational complexity of mining in the Ethereum network, it is practically impossible for an individual running a personal computer to find new blocks. For this reason, mining is performed either in powerful clusters or, even more often, in mining pools. The latter are discussed in \S\ref{subsection:miningpools}.

Finally, PoW is not the only possible consensus algorithm and the Ethereum developers are intensively researching other options, e.g. Proof-of-Stake, which this paper will not cover. The main reason for switching to another strategy is the environmental threat the PoW causes due to the enormous amount of electricity\footnote{https://digiconomist.net/ethereum-energy-consumption} consumed by the mining instances.


%\subsection{Information propagation}
%\label{subsection:infoPropag}

%The efficiency of the Ethereum platform largely depends on the time it takes for transactions to propagate from users to miners and the time it takes for a transaction to get committed \cite{**}.\jpb{we need to define commit.} \jpb{can't we state the same thing about block propagation time?}

%In general, the transaction flow is the following:
%when any Ethereum participant decides to create a new transaction, it broadcasts it to all neighboring peers they are connected to. \jpb{you should have said that peers are connected to K neighbors, and summarize how those connections are set up.}

%A miner includes the transaction into a new block only if: its parameters are valid, the funds are sufficient, the signatures match and if the miner finds the offered fee to be profitable for them. \jpb{you haven't said anything about funds, signatures and mining fees before. you should, otherwise this sentence will not be clear.}

%Finally, miners propagate the transaction back to the network inside a newly mined block. %The Ethereum protocol supports direct whole block messages as well as light new-block announcements that
%After receiving the new block, each peer verifies whether the block's nonce leads into some specific mixHash. Then they verify and execute the individual transactions and synchronize so with the Ethereum platform.\jpb{need to define nonce, mixHash.}


\subsection{Mining Pools}
\label{subsection:miningpools}

The increasing popularity and market capitalization of Ethereum over the years led to a increase in the number of miners.
While this is generally good, as more miners make the network more secure and harder to attack, it also means that the mining difficulty needs to increase proportionally to the mining power in the network.
The downside of this increase in mining difficulty is that regular miners, who use commodity hardware at home, have more difficulty in successfully mining a block and collecting the respective rewards.
Mining pools address this problem by congregating the mining power of multiple users into a single entity.
A typical mining pool consists of a private network running a control server that splits and distributes the workload among individual miners. The workload consists of a Merkle root of a set of transactions and a range of nonces to search through.
The individual participants of mining pools skip the validation phase and solve just a \emph{subpuzzle} of the full cryptographic puzzle, with a lower difficulty.
When a participating miner finds a solution for the puzzle, he sends it to the server, which uses that information to generate the final block and propagates it to the Ethereum network.
The miners are later rewarded in proportion to the computational resources they spent. %The pool typically charges a fee of around one percent\footnote{https://www.cryptocompare.com/mining/\#/pools}.


Currently, there are growing concerns about the power of mining pools on the Ethereum network.
As a matter of fact, just four mining pools control $\approx 70\%$ of Ethereum's total mining capacity which poses some threats to the network security as we will discuss below~\cite{ethPool}. 
Moreover, in our study, we also found evidence that mining pools have been able to mine a large sequence of consecutive blocks which raises concerns about the wisdom of waiting just for 12 confirmation blocks before considering a block as final.

\subsection{Security}

%\subsubsection{Platform security}

% no 50%-miner assumption
The security of the Ethereum platform depends on the assumption that no miner, mining pool, or colluded set of miners, is more powerful than the rest of the network, as that would enable that miner to replace recent blocks and perform double-spending of funds, among other attacks.
It is believed that this assumption is realistic as long as: i) miners are rational, i.e., it is more profitable for them to follow the protocol than to attack it, and ii) miners do not join pools that are too powerful~\cite{Luu2017}.
The intuition is that if miners did that it would make a successful attack trivial (for instance if all miners joined the same pool, that pool could censor transactions and rewrite the blockchain), thus hindering the trust in the platform and making the value of the Ether currency decline.


From the perspective of the end users, and assuming that miners remain rational, the main concern is the issue with block finality discussed above.
It is important to mention that transactions may never commit. 
First, miners can  refuse, for any reason, to include a transaction in a block. Second, even after getting included in a block, that block may not become part of the main blockchain. One can be sure that a transaction will never commit when another transaction from the same account with the same nonce gets committed.
We will discuss these behaviors, among other in \S\ref{Analysis}. 

%\subsubsection{Commit of transactions}
%The existence of forks and the uncertainty about which block will eventually become the part of the main blockchain leads to the need to wait for 12 confirmation blocks to consider a transaction committed.
%The creators of Ethereum argue that this number of blocks~\footnote{https://ethereum.stackexchange.com/questions/183/how-should-i-handle-blockchain-forks-in-my-dapp/203\#203} is sufficient to guarantee the near impossibility to replace such blocks.
%
%







% SKIP   AS   IT   DOES   NOT   RELATE  WITH OUR PAPER
%\subsubsection{End user security}
%The security of funds allocated on Ethereum accounts rely on elliptic curve cryptography which is generally perceived as unbreakable\footnote{TODO Add citation - NSA ref doc} on contemporary computers.
%Therefore, as long as the end users keep their private keys protected, they should not have to worry about an attack breaking the cryptography.



==> cat-future-work-plan.tex <==
\section{Ongoing PhD work}
\newcommand{\docname}{work}
\newcommand{\name}{novel algorithm}
\newcommand{\model}{hybrid consistency}
\newcommand{\nameendAGTattack}{forced fork attack}
\newcommand{\listA}{\emph{maybe-admitted}}
\newcommand{\listB}{\emph{inadmissible}}

\label{sec:concludedwork}
%\subsection{Hybrid consistency model}
The strongly consistent, yet high-latency, commit guarantees of PoW consensus
are inappropriate for many geo-distributed applications.
Further, our experiment suggests this high latency is increasing, as
applications are expected to need to wait for more confirmation blocks for security.
To mitigate this problem, our ongoing work focuses on 
a novel algorithm that extends blockchains 
with an additional weakly-consistent view of the replicated ledger.
This view has a significantly lower latency than current commit
views of existing blockchain systems, while offering a censorship-free 
and causally-correct ledger.
%, which handles conflicts consistently. 
%For many geo-distributed applications, 
The weakly-consistent ledger is a fast path to support those operations of an 
application that do
not require strong consistency.
We are designing it as a pluggable extension
to existing blockchains such as Bitcoin and Ethereum.
\iffalse % begin comment out
\subsection{Improved gossip-based transaction dissemination}
\label{sec:cat:probbcast}
In the first stage of developing our novel algorithm, 
we assumed the existing Ethereum transaction dissemination
protocol is able to reach all nodes in the system within a bounded time
with high probability. However, %this protocol suffers in practice from several deficiencies, 
%such as %high latency for a number of nodes ~\cite{Sirer2018} and 
transactions may not reach
every node when broadcast~\cite{OnAvailability--01}, which may 
compromise this assumption. 
To overcome this problem, we intend to improve the existing Ethereum
probabilistic gossip-based dissemination protocol. %, in \S~\ref{sec:alg:attacks}. 
%Upon inspection of the existing Ethereum transaction dissemination
%protocol implementation in Geth, we observed it uses a variant of \textit{eager push}~\cite{leitao2010gossip}, where nodes send the full
%transaction payload to all their neighbors (as opposed to the standard eager push, 
%where a random subset of known nodes is selected), 
%and on the \textit{infect and die} model~\cite{eugster2004epidemic}, where nodes
%disseminate a transaction upon seeing it for the first time, but take no further action when
%receiving duplicates.	
%We will implement changes to the existing protocol, incorporating concepts from
%previous work like EpTO (Epidemic Total Order)~\cite{Matos2015}
%and including parameters such as peer fanout, number of times an event needs to be relayed and time
%between event relay rounds, which can be adjusted to the characteristics of a given deployment. 
%As a consequence, nodes may be required to connect to more neighbors to increase peer fanout 
%and an increased number of dissemination messages being sent to the network is anticipated
%(due to flooding from eager push, for generating message redundancy~\cite{leitao2010gossip}), 
%after adjusting the relevant parameters. We expect this to allow us to fulfill the goal of reaching all nodes 
%within AGT with high probability, by decreasing transaction dissemination latency and transaction loss.
%Further, Leit{\~a}o \textit{et. al}~\cite{leitao2010gossip} stated that using TCP in a gossip protocol allows using 
%more conservative values for fanout than traditional UDP systems. 
%Ethereum already uses TCP in its gossip protocol and we will also keep using it due to its lower fanout.
%Frey \textit{et. al}~\cite{frey2010boosting} described how Byzantine nodes can attack gossip: i) attack the peer sampling; ii) pollute the protocol %to decrease performance and 
%to increase load on all nodes and lead to a DoS. We will attempt to make our protocol resilient to such attacks.
% paulo: fica a faltar talvez dizer que os trabalhos anteriores eram para ambientes do tipo crash e que o nosso e' bizantino
%We expect this implementation to be pluggable to other blockchain platforms.

%After the implementation, we will measure the network usage impact of the resulting algorithm. 
% weaker reliability of the transaction delivery protocol
%We will also evaluate how \name will behave in scenarios in which the intended probabilistic guarantees are not possible,
%or are too costly.
%To that end, we will run experiments with more challenging network conditions such as
%very high latency (i.e., transaction delay resulting in transactions being placed in the \listA and \listB lists
%or being discarded) and message loss (i. e., transactions and blocks not delivered to all nodes).
\fi % end comment out
%\subsection{Adding hybrid consistency to smart contracts}

%An important fraction of applications that can benefit from our novel algorithm are
%developed by interacting with Ethereum smart contracts. 
We plan to study the integration of our hybrid 
consistency model into smart contract languages like EVM assembly or Solidity \cite{Luu2017}.
%Currently, when externally invoking a method for querying a smart contract
%value (that is, a method that returns a value but does not change any
%internal variables), the returned value reflects the last executed transaction
%that changed the smart contract state. We can consider this transaction
%as \textit{committed}, if it is present in a block that already had $C$ subsequent
%blocks produced after it, or as \textit{uncommitted} otherwise. This is a problem
%for such applications, since they are not aware of the consistency
%guarantees that are offered for the returned value and may be relying on an
%uncommitted value.
We intend to fill this gap by explicitly allowing applications to request a
desired consistency level for the returned value, when invoking such smart
contract methods. 

%Namely, applications will be able to request the 
%following consistency levels:
%\begin{enumerate}
%	\item \textit{Legacy}: Provides the same value as Ethereum today, that is, the
%	value corresponding to the last transaction in a block that changed the corresponding
%	smart contract state.
%	\item \textit{Admitted}: Provides the value resulting from the last admitted transaction that changed
%	the corresponding smart contract state, respecting \model. 
%	This transaction may not have yet been included in a block and it may be ephemerally executed 
%	(i.e., executed to a temporary memory space without becoming permanent).    
%	\item \textit{Committed}: Provides the value resulting from the last committed transaction
%	that changed the corresponding smart contract state. More recent transactions changing this state
%	may already have been executed, but the returned state must not reflect them. It should
%	reflect transactions with $C$ blocks after them.
%\end{enumerate}

%To provide these consistency levels, we anticipate a new layer between
%the smart contract external invocation and the global Ethereum smart contract state.

%For the \textit{Admitted} consistency level, whenever a smart contract method for querying a value is
%invoked requesting this consistency level, we will retrieve all the admitted transactions
%that have not been executed and will execute them in the Ethereum Virtual Machine~\cite{Evm2018}. The
%resulting state will be stored in a temporary memory space instead of becoming permanent and 
%will be used when executing the invoked method.

%For the \textit{Committed} consistency level, we will also store the previous global state that would result 
%from not having executed the last $C$ blocks.  Thus, whenever a smart contract method that queries a value is
%invoked requesting this consistency level, this previous global state will be used.


%\subsection{Weaker probabilistic assumptions}

%We plan to study, both formally and empirically, what is the impact 
%that weaker probabilistic assumptions (namely, the  
%reliability of the transaction delivery protocol and the guarantees of PoW commit)
%effectively have on probabilistic guarantees provided by \name.

%% weaker reliability of the transaction delivery protocol
%In \S~\ref{sec:cat:probbcast}, we proposed improving the blockchain dissemination components
%with more reliable probabilistic guarantees. Nonetheless, it is important to assess how
%\name will behave in scenarios in which such probabilistic guarantees are not possible.
%We will thus try to run experiments with more challenging network conditions such as
%very high latency (i.e., transaction delay resulting in transactions being placed in the \listA and \listB lists
%or being discarded) and message loss (i. e., transactions and blocks not delivered to all nodes).

%% weaker guarantees of PoW commit
%We have previously considered a transaction $t$ as \textit{committed} after $C$ blocks have been 
%produced after a block including $t$, using PoW. 
%However, this is a probabilistic assumption, which means that theoretically
%a malicious user could produce a chain that is slightly longer than $C$ (with very low probability). 
%We will try to assess how \name behaves when the PoW guarantees are not met (i.e. when more than $C$
%blocks are replaced).

%Previous work has set a theoretical limit on the minimum block time without risking security and related it with the
%block transmission time \cite{Kiayias2015speed}. We will try to assess the effect of reducing block size in \name,
%when attempting to minimize the block time and consequently improve the commit time.

%\subsection{\model with no PoW}

%Another direction is to study how the \model could be used without requiring PoW.
%We will evaluate whether \name could be used with blockchains using emerging 
%alternatives to PoW, such as Byzantine Agreement (BA) protocols, Proof-of-Stake (PoS) \cite{Berger2018} and Proof-of-Space (PoSp) \cite{Kiayias2017}.
%The \textit{committed} guarantee will have to be provided using the corresponding guarantees
%in those technologies.  As an example, the Algorand blockchain has been described as confirming transactions on the
%order of a minute, with a negligible fork probability \cite{Gilad2017}. Using \name with Algorand can thus mean having even lower commit times
%than with Ethereum on average, in case forks are as negligible as described, and having the \model model available.



%Table \ref{tab:wkplan} presents our workplan.

% https://www.tablesgenerator.com/
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%\begin{table}[!hbt]
%\begin{tabular}{@{}llllllllllll@{}}
%\toprule
%Activity                & 2019                     &                                                 &                          &                          &                                                 &                                                 &                                                 &                                                 & 2020                                            &                                                 &                                                 \\ \midrule
%Probabilistic broadcast & \cellcolor[HTML]{FE996B} & \cellcolor[HTML]{FE996B}                        &                          &                          &                                                 &                                                 &                                                 &                                                 &                                                 &                                                 &                                                 \\
%Smart contracts         &                          & \cellcolor[HTML]{FE996B}{\color[HTML]{F8A102} } & \cellcolor[HTML]{FE996B} & \cellcolor[HTML]{FE996B} & \cellcolor[HTML]{FE996B}                        &                                                 &                                                 &                                                 &                                                 &                                                 &                                                 \\
%Weaker assumption       &                          &                                                 & \cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FE996B} & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } &                                                 &                                                 &                                                 &                                                 \\
%No PoW                  &                          &                                                 &                          &                          &                                                 & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } &                                                 &                                                 &                                                 \\
%Thesis writing          &                          &                                                 &                          &                          &                                                 &                                                 & \cellcolor[HTML]{009901}{\color[HTML]{009901} } & \cellcolor[HTML]{009901}{\color[HTML]{009901} } & \cellcolor[HTML]{009901}{\color[HTML]{009901} } & \cellcolor[HTML]{009901}{\color[HTML]{009901} } & \cellcolor[HTML]{FFFFFF}{\color[HTML]{009901} } \\ \bottomrule
%\end{tabular}
%\vskip 5mm 
%\caption{Work plan}
%\label{tab:wkplan}
%\end{table}



==> intro-docforum.tex <==
%%%%%%%%%%%   INTRODUCTION   %%%%%%%%%%%

\section{Introduction}

%trabalhos anteriores focaram-se num conjunto incompleto de metricas (ou seja, nao cobrindo todos os pilares fundamentais da tecnologia) e na perspetiva de um observador apenas (ou seja, sem visao 'a escala planetaria)

Over the recent years, permissionless blockchains have enjoyed rapid growth and gathered remarkable interest. % -- no longer just from technological enthusiasts, but from the general public as well.
 Permissionless blockchains enable cryptocurrencies and other distributed applications based on smart contracts that promise to
 revolutionize the current payment methods with the
 ambition to eliminate the need for banks or other centralized entities acting as trusted mediators of financial operations. 
% The goal of the technology is to guarantee an honest and proper execution of user transactions that can be verified by anyone that joins the system.
% Furthermore, permissionless blockchains can also support Smart Contracts, which introduce a game-changing paradigm for building new kinds of byzantine fault-tolerant geo-distributed applications~\cite{Yellow,SmarterContracts,ConcurrentPerspective}. 
% These appealing features led to a wide adoption by users resulting in a market capitalization in the order of the thousands of billions of dollars~\cite{marketCap}.

At the core of most permissionless blockchains lies a conceptually simple protocol, such as the Proof-of-Work (PoW) consensus proposed by
Nakamoto~\cite{BitcoinShortened}, which specifies the rules on how the blockchain % underlying replicated ledger 
should grow and converge.
%how the replicated ledger grows and converges consistently.
Despite this simple core mechanism, real-world permissionless blockchain deployments 
such as Bitcoin~\cite{BitcoinShortened} or Ethereum~\cite{Yellow},
are extremely complex systems composed of several modules and protocols whose properties are intrinsically hard to understand.
%To further complicate matters, not all implementations follow the specifications, while different clients have
%different default parameters \cite{Parity2019, Geth17DefaultConfig}. 

%%\jpb{We should revise this list of ``real-world issues'', I just wrote it from scratch, so I may well be missing important points.}
%As a matter of fact, permissionless blockchains protocols coordinate a vast and
%geographically-distributed system of nodes by resorting to epidemic protocols
%whose emerging behavior is inherently probabilistic and hard to model.
%The set of nodes is open by nature, which provides users with a
%considerable margin to behave selfishly or maliciously.
%This adversarial environment is a further obstacle to any attempt to accurately
%understand and predict the emerging characteristics of the system.
Additionally, permissionless blockchains have long evolved from a plain organization composed of individual miners, to an ecosystem dominated by mining pools. % that reorganize the mining resources in complex and opaque ways.
At the time of writing, the top four mining pools have around 60\% and 70\% of Bitcoin's and Ethereum's total network capacity --- the top permissionless blockchains ---
respectively~\cite{btcPoolNoAccess,ethPoolNoAccess}.
Finally, they rely on a large code-base that includes different implementations (and versions) of the software that blockchain nodes and clients run.
It is fundamental to see how they behave, what doesn't work and opportunities for improvement. 

%Given the large adoption and economical impact of blockchains --- which is expected only to grow in the next decade~\cite{gatnerVal} ---, the complexity of the underlying systems, and the adversarial environment in which they operate, it is therefore fundamental to properly study and understand the emergent behavior and properties of these systems. 
Recent work has performed measurement studies of popular
permissionless blockchains~\cite{InfPropagaion--02, OnAvailability--01,
MeasEthPeersShortened, Sirer2018}. Together, these studies have contributed
to a better understanding of how these intricate large-scale systems perform in practice, 
unveiling some findings that were not originally anticipated.
Still, the general picture attained by these studies is inaccurate and incomplete. This is mostly due to some key limitations: 
%(i) previous studies either focus on one or few facets of the whole system~\cite{InfPropagaion--02, OnAvailability--01, MeasEthPeers, Sirer2018}, instead of following a holistic analysis that considers the remaining fundamental facets;
(i) relying on a single observation point, therefore neglecting how the geographical distribution of the network affects such measurements~\cite{InfPropagaion--02, OnAvailability--01};
(ii) not considering the recent predominance of mining pools as first-class components in today's blockchain landscape~\cite{InfPropagaion--02, OnAvailability--01,
MeasEthPeersShortened};
(iii) ignoring transaction commit time and how it can be negatively impacted by network delays, out-of-order transactions and empty blocks
\cite{Sirer2018,MeasEthPeersShortened}.

We start by describing our experience and lessons
learned on implementing and deploying a measurement infrastructure across different
continents, addressing some of the limitations of previous studies.
We focus on the Ethereum blockchain, the second most valuable cryptocurrency. % and the leading decentralized platform for Smart Contracts.
An extended description of our study can be found in \cite{Silva2020}.
%To achieve this, 
We implemented and deployed a measurement infrastructure
consisting of several especially modified Ethereum nodes placed across different
continents.
Our measurement nodes run an instrumented variant of the Geth open-source
implementation of Ethereum clients. Each measurement node can connect to the main network and collect the desired measurements from the transactions and blocks it observes.
We analyzed long-running measurements acquired by four measurement nodes which were
deployed in North America (NA), Eastern Asia (EA), Western Europe (WE) and Central Europe (CE). 

% We use it to perform a long-lasting measurement with the goal of collecting
% and analyzing a wide range of network metrics, as well as examining several
% until now never studied blockchain properties.


We highlight the following key results of our study:
i) We identify the generalized and consistent practice of different forms of selfish behavior that harm the throughput of the main blockchain. To the best of our knowledge, these practices were not documented and/or not empirically studied systematically
before;
ii) We confirm that the geographical location has a relevant impact on block reception times and that the prevalence of powerful mining pools exacerbates such
effect; 
iii) We provide empirical evidence that the standard 12-block confirmation
rule of Ethereum may not provide the strong probabilistic
guarantees on block finality that are usually assumed in literature;
%\item We confirm prior findings that were considered as part of our metrics, now with updated trends.
iv) We confirm that some of the metrics collected by previous works still present the same values and report relevant changes to other such metrics.

% Our study confirms some previously documented findings but from a multi-observer approach.
% Most importantly, our study sheds new light on the characteristics of Ethereum, as of today, with some additional new findings.
% Among others, we highlight the following:


% \begin{itemize}

%   % joao: the following items need to be revised
  
% \item %geo position influence
% To the best of our knowledge, we are the first ones to measure the block propagation delays and to identify that peers placed geographically closer to mining pools synchronize faster.

% \item % min. pools create forks (blocks with the same height) ..
% We find that prominent mining pools exploit the uncle block reward system and intentionally mine outdated blocks.

% \item % censorship
% Finally, we observe that blockchain consists of long sequences of blocks mined by a unique entity, which enables the possibility of transaction censorship. In consequence, we argue that the current rule of thumb of 12-confirmation-blocks waiting time is not sufficient.

% \end{itemize}



% Previous work~\cite{OnAvailability--01} from 2017 studied various  properties
% of the Ethereum platform, such as what impact the user-defined variables
% "gas price" and "gas limit" have on transaction inclusion, the commit time
% of transactions or the ratio of blockchain forks.
% We replicate and verify their measurements in order to observe how the
% properties changed over the last two years.
% Moreover, we take attention at details, that the authors of ~\cite{OnAvailability--01} omitted, such as the relation between fork lengths and the probability of being referenced in main blocks.
% On top of that, we measure various metrics regarding the forked blocks, e.g. the degree of transaction reordering, and add several other metrics, such as the degree of redundant receptions of new block announcements, with the aim to observe the network traffic overhead.

% Although Ethereum has been out and running for several years and a growing body of research has thoroughly studied it, we were missing an analysis of the Ethereum's underlying network concerning the inconsistencies amidst individual nodes and measuring the propagation delays of information.

% In this work, we are interested in measuring and evaluating the network characteristics of the currently second most valuable cryptocurrency, Ethereum.
% Ethereum opearates on an underlying peer-to-peer network protocol which must support the interconnection of a large number of peers spread all over the world, prevent the creation of network partitions, and allow for a smooth transfer of all the data needed in the system.
Our main contributions are the following:
i) A one-month study of the Ethereum network from several geographically dispersed observation
points;
ii) A set of open-source measurement and processing tools that allows other researchers to reproduce our observations and/or perform similar studies in other blockchain
systems;
iii) The collected data set which might enable other researchers to do other findings in our collected data or refine our
observations. %\footnote{For double-blind purposes both the code and the data set is currently withheld. We will make both publicly available to the community.}

%Briefly, we rely on a multi-observer approach in which our measurements were obtained at multiple geographically-dispersed observer nodes.
%This allows us to 
%We assess the impact of the geographic location in key metrics. 
%For instance, we show that block propagation time is highly skewed, allowing peers in some regions to observe first a large portion of the total blocks --- which gives them a competitive advantage when mining.
%We leverage these multiple observation points to assess the key pillars of Ethereum, namely network efficiency (\S\ref{subsec:netEff}), geographical dispersion (\S\ref{subsec:geoImpact}), blockchain efficiency (\S\ref{subsec:blockchainEff}) and security (\S\ref{subsec:sec}), and the impact mining pools have on each of these.


%The remainder of this paper is organized as follows.
%\S\ref{bg} provides essential background on permissionless blockchains in general and Ethereum in particular.
%\S\ref{methodology} describes our measurement infrastructure and methodology.
%\S\ref{Analysis} presents the main results of our study, while
%\S\ref{relwork} provides essential related work.
%\S\ref{Lessons} describes the lessons learned from our results
%and proposes lines for mitigating the major threats that our study identified.
%Lastly, \S\ref{conclusions} draws our final conclusions.


==> lessonslearned.tex <==
%%%%%%%%%%%   LESSONS LEARNED   %%%%%%%%%%%
\section{Lessons learned}
\label{Lessons}
% strengths, challenges and surprises 
Our experiment shed light on strengths and challenges of the Ethereum network, while offering some surprises.
The low propagation delay we observed can be considered a strength of the Ethereum network.
In contrast, mining pool centralization can lead to challenging and surprising selfish behaviors. 
% previous text
Commit delays in Ethereum have been improving relatively to the delays reported in prior studies, which can be mostly explained by the adoption of
shorter inter-block times in Ethereum \cite{Etherscan2019}.
Still, we identified selfish behaviors that may place real threats to the
throughput of the system -- most notably, empty blocks and one-miner forks.
They all represent distortions of the incentive model of Ethereum, which
encourage selfish nodes to waste system resources (namely, mining power
and network capacity) in
intentional efforts that do not contribute to the progress of the main
blockchain.
To the best of our knowledge, these behaviors were not anticipated in the
original design of the system \cite{Yellow}. Hence, current implementations
tolerate them.
While our study found relatively scarce occurrences of such
selfish behaviors, with a low impact on the overall throughput of the system,
they were observed consistently over the experiments.
This suggests that these behaviors are profitable to selfish nodes,
hence there is a risk that the frequency and impact of such situations
grows in the future.

% same miner uncle blocks
Regarding one-miner forks, we argue that the Ethereum protocol should forbid referencing uncles mined by miners that have already mined a main block of the same height. This would -- as our results show -- save around 1\% of the platform's overall computational resources which are currently spent on mining forks, while at the same time giving a higher chance that small miners collect those rewards. The uncle block rate of a mining pool would be effectively slowed down, even if the mining pool tried to use distinct coin addresses for claiming the rewards, since mining power would be split among those addresses. Additionally, we have observed that, in 56\% of cases, mining pools appeared to be using their full mining power for mining distinct versions of the same block (i.e. with the same transaction set) with the same height. In the remaining 44\% of the cases, they were mining different blocks (i.e. with distinct transaction sets) with the same height. This means our solution would effectively deter mining pools from using their full mining power to mine distinct versions of the same block, in more than half of the one-miner fork cases.
%In one-miner forks, uncle block rewards are being exploited by mining pools, rather than helping small miners. To mitigate
%this problem, such uncle blocks should be rejected by the network. 
Further, producing such blocks could be considered a protocol violation and a miner could be punished by having funds removed from his coinbase account~\cite{xiao2019survey}.
% empty blocks
%To prevent empty blocks from harming the system throughput in the future, mining them could be disallowed or their reward could be so small that mining them would not pay off.
A robust solution to put an end to empty blocks should be designed,
to prevent them from harming the system throughput.
However, this is a challenging endeavor that is left for future work.

Our study also highlights that the emergence of mining pools has rendered
some initial design assumptions \cite{Buterin2015} obsolete today.
Among multiple findings of our study that support this claim,
we observed that the usual 12-block
confirmation rule of Ethereum may not provide the strong probabilistic
guarantees that are promised by probabilistic
analysis that unrealistically rely on a flat and large universe of
individual miners.
More concretely, we observed that the centralization of most mining power on
Ethereum has already enabled alarmingly long sequences of consecutive blocks
(lengths of 8, 9 and even 14 blocks) generated by a single mining pool. This emphasizes that, for permissionless blockchain protocols whose design
allows mining pool-like extensions, these need to always be considered
as first-class elements of the ecosystem at the earliest design stages.
%This not just true in the context of Ethereum, but also in the context of
%any blockchains whose design allows mining pool-like organizations of the
%mining power.
However, we observe that the underlying system model considered by many
research papers that study or propose new blockchain implementations
% (e.g., \cite{***some examples***})
omits mining pool organizations from
their underlying system models ~\cite{InfPropagaion--02, OnAvailability--01, MeasEthPeers}. This common practice should be avoided by the research community.
\jpb{it would be cool if we supported the above sentence with concrete citations to papers that are examples of this practice. However, probably we don't have the time for that.}


% key trends changed 
Our study also %evisited some previously studied facets of Ethereum, and
revealed that some key trends changed in a short time span, such as: 
i) the median waiting time for 12 blocks decreased from 200 seconds to 189 seconds~\cite{OnAvailability--01};
ii) a substantial increase in out-of-order committed transactions from 6.18\% to 11.54\%~\cite{OnAvailability--01};
iii) the proportion of forked blocks increased by more than 1\% and fork lengths increased as well.
This confirms that large-scale permissionless blockchain systems % (such as Ethereum) 
are eminently dynamic, and highlights the importance of
studies like ours to take place regularly. We make our tools available to encourage this.
Finally, we have systematically confirmed that the geographical location of
a node has a consistent impact on the level of service that node gets from the
system. More than a symptom that the set of nodes is not evenly spread across
the globe, this reflects the fact that a large portion of Ethereum's activity now
 depends on a small and poorly dispersed subset of nodes that comprises the gateways of the major mining pools.
 This stresses the importance of multi-observer measurement approaches when characterizing permissionless blockchains, as followed by our study.
 %We hope that the open-source availability of our measurement tools will help future studies fulfill this recommendation.
 %% those aspects that are influenced by this topological trends.
 


==> methodology.tex <==
%%%%%%%%%%%   METHODOLOGY   %%%%%%%%%%%
\section{Methodology}
\label{methodology}

In this section, we describe our methodology.
Recall that our goal is to assess the emerging behavior of Ethereum according to several key aspects, namely: the impact of geographical dispersion, network efficiency, blockchain efficiency, security, and the impact mining pools have on each of these.
To achieve this, we created a modified Ethereum client that collects the metrics of interest and deployed it over three continents.
We used Geth version $1.8.23$ as the basis for our measurements. %\footnote{https://github.com/ethereum/go-ethereum/releases/tag/v1.8.23}.
The rationale behind choosing Geth in favor of the other available client implementations is that Geth is Ethereum's reference implementation
and the most widely used client, with more than 74\% of the user share\cite{Ethernodes2019}. The client was instrumented to capture and log all incoming network messages, hence allowing us to collect information about incoming transactions, blocks, and peer connection requests.
Each measurement is logged to a dedicated log file together with a local timestamp.
%Note that we timestamp the measurement at the exact moment of message arrival, before any message validation or processing is done, in order to minimize the measurement error but also to capture invalid messages that would otherwise be discarded by the validation logic.
%Because the logs can grow very fast, we rely on \texttt{syslog}\cite{syslog} to manage log rotation and compression. 
We collected 600 GB of raw logs and analyzed them using \textit{pandas} \cite{Pandas2019} and \textit{NumPy} for Python \cite{NumPy2019}.

Our modifications to Geth entailed adding and adapting roughly 1,000 lines of code.
We used Geth's default settings  except for the number of peers we can connect to, which we set to unlimited in order to observe as much information from the network as possible.
%This is because we wanted to observe as much information as possible. 
%Second, we set the minimum gas price of incoming transactions to zero, in order to not discard underpriced transactions.
These settings are identical to the measurement client configuration used in Weber et al.~\cite{OnAvailability--01}, which allows us to compare our results with theirs.
Note that, apart from the instrumentation effort and the number of connected peers, no other changes have been made to Geth --- in particular, our client behaves like any other client in the network and thus it is indistinguishable from any other regular client.
This is fundamental to obtain unbiased results.




%We deployed the measuring peers on our infrastructure consisting of four computing instances, three of them were rented virtual machines located in Eastern United States, Eastern Asia, and Central Europe.
%The fourth instance was a dedicated multicore computer located in Western Europe.

The instrumented version of Geth was deployed in computing instances located in North America, Eastern Asia, Western Europe and Central Europe. 
They were connected directly to the Internet backbone with a network throughput of at least 8 GB/s. 
A detailed description of the specification of each machine can be found in Table~\ref{tab:machines}.
These specifications are well above the minimum requirements to run an Ethereum client so we do not expect any biases due to poor hardware performance~\cite{ethBook}. 
Each machine used the Network Time Protocol (NTP) %over the Internet 
for clock synchronization. NTP provides offsets lesser than 100ms in 99\% of cases and lesser than 10ms in 90\% of cases\cite{NTP}.
%As we will discuss in \S\ref{Analysis}, this NTP precision places a constraint on the measurement errors of our observations

Part of our study involves analyzing propagation delays
in the Ethereum network, with a particular focus on blocks.
%One naive approach to measure these would be to compare the time
%at which a block is received at a measurement node with the
%timestamp that each block carries, which are set by the miner that
%generated the block.
%However, this timestamp is unreliable, not only because it can be freely set by the latter node, but also because we cannot make assumptions about the synchronization of those nodes' clocks.
%Therefore, 
We adapt the method proposed by Decker et al. \cite{InfPropagaion--02}, which exclusively relies on timestamps generated by our measurement nodes to compute the block propagation delay. More precisely, we define the propagation delay of a block as the time difference between the first observation of that block at any instance of a measurement node and the times of arrival on the remaining measurement nodes. 
Note that this is an approximated method since (i) it does not measure the time it takes to propagate a
transaction or block from the miner
to the first measurement node that received that block; and (ii) the accuracy of our measurements is always bounded by the accuracy of NTP. % in synchronizing the local clocks of our measurement nodes.
%Hence, hereafter we use this method when the measured block propagation delays being analyzed have a much higher amplitude than the above-mentioned inaccuracy.
We take this limited accuracy into consideration whenever relevant.
% We also note that this inaccuracy is generally not acceptable for transaction delays, which are short and thus typically propagate at a low latency.




%The parameters of the machines are presented in Table~\ref{tab:machines}.

\begin{table}
\begin{tabular}{m{1cm} m{3.2cm} m{1cm} m{1cm}}
\hline
Location & CPU & RAM (GB) & Bandwidth (Gbps) \\
\hline
NA  & 4x  Intel~Xeon~2.3~GHz & ~~15    & ~~8   \\
EA  & 4x  Intel~Xeon~2.3~GHz & ~~15    & ~~8   \\
CE  & 4x  Intel~Xeon~2.4~GHz & ~~~8    & 10  \\
WE  & 40x Intel~Xeon~2.2~GHz & 128    & 10  \\ \bottomrule
\end{tabular}
\caption{Specifications of the measurement infrastructure.}
\label{tab:machines}
%\vspace{-1.2cm}
\end{table}

%    	{US}  & {Intel~Xeon~2.3~GHz}  & 4  & {15 GB}  & {370 GB}  & {Debian 9} & {8 Gb/s}  \\
%    	{EA}  & {Intel~Xeon~2.3~GHz}  & 4  & {15 GB}  & {370 GB}  & {Debian 9} & {8 Gb/s}  \\
%    	{CE}  & {Intel~Xeon~2.4~GHz}  & 4  & {8 GB}   & {$500$ GB}  & {CentOS 7} & {10 Gb/s}  \\
%    	{WE}  & {Intel~Xeon~2.2~GHz}  & 40 & {128 GB} & {$1,000$ GB} & {Ubuntu 18.04} & {10~Gb/s}   \\ \bottomrule

% virt. machines    |  PT (40cores)
% 100 - 150 peers   | 200+peers at any moment,

We performed the measurements from April 1\textsuperscript{st} 2019 to May 2\textsuperscript{nd} 2019, with each machine connected to more than 100 peers at any moment.
Additionally, we did a complementary measurement on the WE instance with the default number of 25 peers. 
This measurement was meant to capture the behavior of an Ethereum client with default settings and took place from May 2\textsuperscript{nd} to May 9\textsuperscript{th}.
\textit{Ethical Considerations:} The machines and Geth client we deployed follow exactly the Ethereum protocol rules and thus have no negative impact on the behavior of the Ethereum network.
The data we collected is publicly available to anyone that connects to the Ethereum network and therefore it does not raise privacy concerns.


%Our measurements were ethically sound, as our instances complied with the Ethereum protocol rules and thus did not pose any negative impact on the behavior of the Ethereum network during our measurements. 



==> ref_shorten.tex <==
\begin{thebibliography}{00}
\bibitem{asymsched} B. Lepers et al. Thread and Memory Placement on NUMA Systems: Asymmetry Matters. USENIX ATC'15.
\bibitem{batman} C. Chou et al. BATMAN: Techniques for Maximizing System Bandwidth of Memory Systems with stacked-DRAM. MEMSYS'17.
%\bibitem{lamport94} Leslie Lamport. A Document Preparation System.
\bibitem{smart_arrays} I. Psaroudakis et al. Analytics with Smart Arrays: Adaptive and Efficient Language-independent Data. EuroSys'18.
\bibitem{estima} G. Chatzopoulos et al. ESTIMA: Extrapolating ScalabiliTy of In-Memory Applications. ACM Trans. Parallel Comput. 2017.
\bibitem{nas} D. H. Bailey et al. The NAS Parallel Benchmarks\&Mdash;Summary and Preliminary Results. Supercomputing'91.
\bibitem{splash} S. C. Woo. The SPLASH-2 Programs: Characterization and Methodological Considerations. ISCA'95.
\bibitem{carrefour} M. Dashti et al. Traffic Management: A Holistic Approach to Memory Placement on NUMA Systems. ASPLOS'13.
\bibitem{memorycontroller} Z. Majo et al. Memory System Performance in a NUMA Multicore Multiprocessor. SYSTOR'11.
\bibitem{BA-ics} S. Yu et al. Design and Implementation of Bandwidth-aware Memory Placement and Migration Policies for Heterogeneous Memory Systems. ICS'17.
\bibitem{} S. Kaestle et al. Machine-aware Atomic Broadcast Trees for Multicores. OSDI'16
\bibitem{numactl} Andi Kleen. numactl(last accessed: 28/03/2018). \url{https://linux.die.net/man/8/numactl}.
\bibitem{memprof} R. Lachaize. MemProf: A Memory Profiler for NUMA Multicore Systems. USENIX ATC'12
\bibitem{lira} A. Collins et al. LIRA: Adaptive Contention-Aware Thread Placement for Parallel Runtime Systems. ROSS'15
\bibitem{Sched-NUMA} AutoNUMA: the other approach to NUMA scheduling (last accessed: 2018-01-10). \url{https://lwn.net/Articles/486858/}. 
\bibitem{ptmalloc} W. Gloger. A fast, memory-efficient implementation of malloc for Unix systems (last accessed: 2018-28-03). \url{http://www.malloc.de/en/}.
\bibitem{memory-access-pattern} Z. Majo et al. Matching Memory Access Patterns and Data Placement for NUMA Systems. CGO'12.
\bibitem{numa} C. Lameter. NUMA (Non-Uniform Memory Access): An Overview. ACM Queue, 2013.
\bibitem{nucore} W. Wang et al. Predicting the memory bandwidth and optimal core allocations for multi-threaded applications on large-scale NUMA machines. HPCA'16.
\bibitem{lapt} E. H. M. Cruz et al. Optimizing Memory Locality Using a Locality-Aware Page Table. SBAC-PAD'14
\bibitem{kernel-based} M. Diener et al. Kernel-Based Thread and Data Mapping for Improved Memory Affinity. IEEE Transactions on Parallel and Distributed Systems, 2016. 
\bibitem{parsec} Christian Bienia. Benchmarking Modern Multiprocessors. Princeton University, 2011.
\bibitem{Buss:1987:VTB:897367} Andreas Kleen. A numa api for linux. Technical Linux Whitepaper, 2005.
\bibitem{pandia} D. Goodman et al. Pandia: Comprehensive Contention-sensitive Thread Placement. EuroSys'17.
\bibitem{shoal} S. Kaestle. Shoal: Smart Allocation and Replication of Memory for Parallel Programs. USENIX ATC'15.
\bibitem{dramon} W. Wang et al. DraMon: Predicting memory bandwidth usage of multi-threaded programs with high accuracy and low overhead. HPCA'14.
\bibitem{mctop} G. Chatzopoulos et al. Abstracting Multi-Core Topologies with MCTOP. EuroSys'17. 
\bibitem{gpu} N. Agarwal et al. Page Placement Strategies for GPUs Within Heterogeneous Memory Systems. ASPLOS'15.
\bibitem{mongodbnuma} The MongoDB 4.0 Manual. (last accessed: 2018-01-10). \url{https://docs.mongodb.com/manual/administration/production-notes/}.
\bibitem{mysqlnuma} MySQL Bugs, Bug \#57241. (last accessed: 2018-01-10). \url{https://bugs.mysql.com/bug.php?id=57241}.
\bibitem{cassandranuma} AWS Cassandra: Cassandra, NUMA and EC2. (last accessed: 2018-01-10). \url{http://cloudurable.com/blog/cassadra-numa-ec2-aws/index.html}.
\bibitem{mbind} mbind - set memory policy for a memory range. (last accessed: 2018-01-10).\url{https://linux.die.net/man/2/mbind}.
\bibitem{mbind} numa - NUMA policy library. (last accessed: 2018-01-10).\url{https://linux.die.net/man/3/numa}.
\bibitem{memory_performance} D. Patterson et al. A Case for Intelligent RAM. IEEE Micro'97.
\bibitem{callisto} T. Harris. Callisto: Co-scheduling Parallel Runtime Systems. EuroSys'14.
\bibitem{denoyelle:hal-01622582} N. Denoyelle et al. Modeling Large Compute Nodes with Heterogeneous Memories with Cache-Aware Roofline Model. PMBS'17
\bibitem{Mohtasham:2016:ROP:2935764.2935770} A. Mohtasham et al. RUBIC: Online Parallelism Tuning for Co-located Transactional Memory Applications. SPAA'16
\bibitem{Majo:2017:LPC:3057718.3040222} Z. Majo et al. A Library for Portable and Composable Data Locality Optimizations for NUMA Systems. ACM Trans. Parallel Comput. 2017.
\bibitem{Georgakoudis:2017:SSP:3154814.3158643} G. Georgakoudis et al. SCALO: Scalability-Aware Parallelism Orchestration for Multi-Threaded Workloads. ACM Trans. Archit. Code Optim.2017
\bibitem{Cho:2016:OSC:2967938.2967960} Y. Cho et al. Online Scalability Characterization of Data-Parallel Programs on Many Cores. PACT'16
\bibitem{Pusukuri:2015:TEL:2836331.2827698} K. K. Pusukuri et al. Tumbler: An Effective Load-Balancing Technique for Multi-CPU Multicore Systems. ACM Trans. Archit. Code Optim. 2016.
\bibitem{Zhao:2016:COP:2967938.2967939} Y. Zhao et al. Characterizing and Optimizing the Performance of Multithreaded Programs Under Interference. PACT'16.
\bibitem{Prekas:2015:EPW:2806777.2806848} G. Prekas et al. Energy Proportionality and Workload Consolidation for Latency-critical Applications. SoCC'15.
\bibitem{Harris:2015:CFP:2813767.2813771} T. Harris et al. Callisto-RTS: Fine-grain Parallel Loops. USENIX ATC'15.
\bibitem{Srikanthan:2016:CSL:3026959.3026989} S. Srikanthan et al. Coherence Stalls or Latency Tolerance: Informed CPU Scheduling for Socket and Core Sharing. USENIX ATC'15.
\bibitem{Zhuravlev:2012:SST:2379776.2379780} S. Zhuravlev et al. Survey of Scheduling Techniques for Addressing Shared Resources in Multicore Processors. ACM Computing Survey, 2012.
\bibitem{dino} S. Blagodurov et al. A Case for NUMA-aware Contention Management on Multicore Systems. USENIX ATC'15.
\bibitem{tech-report-parallel-computing} K. Asanović et al. The Landscape of Parallel Computing Research: A View from Berkeley. University of California, Berkeley. 2006.
\bibitem{copart} J. Park et al. CoPart: Coordinated Partitioning of Last-Level Cache and Memory Bandwidth for Fairness-Aware Workload Consolidation on Commodity Servers. EuroSys'19.

\end{thebibliography}

==> related-work.tex <==
\section{Related work}
\label{relwork}
%In this section we discuss the body of work that has focused on analyzing one or more aspects of permissionless blockchains, namely Bitcoin and Ethereum.

A body of work has studied decentralization, the key distinctive feature of blockchain with respect to more traditional centralized approaches, and an important property for high resistance against censorship of individual transactions~\cite{Sirer2018, Luu2017, eyal2018majority, miller2015discovering}. 
Luu \textit{et. al}~\cite{Luu2017} reported that around 80\% of the mining  power in Ethereum resides in less than ten mining pools, which is corroborated by our observations.
Gencer \textit{et. al}~\cite{Sirer2018} showed that both Bitcoin and Ethereum suffer from a centralized mining process, due to mining pools. Miller \textit{et. al}~\cite{miller2015discovering} showed that 75\% of the mining power in Bitcoin resides in just 2\% of the nodes.
Eyal and Sirer~\cite{eyal2018majority} described an attack to Bitcoin preventing decentralization, in which rational miners prefer to join the selfish miners and the resulting colluding group becomes a majority.
% our results
Our observations confirm these hypotheses and show that Ethereum mining pools have the power to temporarily censor transactions and harm their commit time by mining long sequences of blocks.

% waiting 12 blocks
Previous research has focused on the time it takes for a transaction to commit~\cite{OnAvailability--01, Bitcoin, Buterin2015}. 
Nakamoto~\cite{Bitcoin} showed the probability of not replacing a Bitcoin block $B$ containing transaction $t$ with a malicious block $B'$ without $t$ can be made arbitrarily high, whereas Buterin \cite{Buterin2015} studied the corresponding probability for Ethereum. 
In Bitcoin, the probability that is deemed \emph{safe} is achieved after 6 blocks, corresponding to one hour, whereas in Ethereum this is achieved after 12 blocks, corresponding to around 3 minutes~\cite{OnAvailability--01}.
In our one-month observations we observed two instances where a single mining pool was able to mine 9 consecutive blocks twice, and we also observed that over all the blocks ever mined, a mining pool was able to mine a sequence of 14 consecutive blocks.
This means that mining pools are indeed able to censor transactions and rewrite the blockchain, and therefore should raise concerns about the security of the network. %As a future research direction, transaction censorship resistance could be added to Ethereum. 
%A short term solution to this problem would be increase the number of confirmation blocks from 12 to 15, which is higher than the longer sequence ever observed.
%The downside is that such increase would result in an increase in latency of around 45 seconds (i.e. three additional blocks at an average of 15 seconds per block).
%The long term solution is, in our opinion, to create incentives that reward small or individual miners.
%This is, however, very challenging because mechanisms such as the uncle blocks that were introduced to incentivize small miners, can end up being exploited by the mining pools themselves as we observed during our measurements.

%This high probability comes at the price of waiting on average about one hour for 6 blocks, in Bitcoin, and waiting on average about 3 minutes for 12 blocks, in Ethereum~. 
%Our work observed that a single mining pool can actually mine sequences of more than 12 blocks in Ethereum, which may compromise its security.

%% transaction reordering/blockchain anomaly
%Natoli and Gramoli~\cite{Natoli2016} described the \textit{Blockchain anomaly}, which may prevent blockchains from executing dependent transactions in the correct order, due to forks. They argued that PoW blockchains do not ensure consensus safety deterministically. Further, Li \textit{et. al}~\cite{Li2017} identified Ethereum Smart Contracts as vulnerable to this problem. 
%In this context, our work analyzed the degree of transaction reordering in forked blocks which is $11.54\%$. 
%This reordering is non-negligible, and seems to be getting worse over time as measurements done two years ago reported a reordering of $6.18\%$, around half of what we observed~\cite{OnAvailability--01}.
%This further demonstrates the dynamic nature of Ethereum, and we argue, that measurements such as those conducted in this paper should be done periodically to better assess the behavior of the system and, perhaps, help guide its development.

%%transaction removal
%Natoli and Gramoli~\cite{Natoli2016balance} also studied double-spending in Ethereum through the \textit{balance attack}, which allows removing an attacker's transaction by replacing a block containing it. Karame \textit{et. al}~\cite{karame2012double} studied a low-cost double-spending attack on Bitcoin fast payments. In our work, we observed that around 2.5\% of transactions were replaced by another transaction with the same nonce from the same account, some of which may represent double-spending attacks.

Previous work attempted to describe the causes of mining empty blocks~\cite{mccorry2018smart, kovst2018transition}. 
%% Goldfinger attack
%McCorry \textit{et. al}~\cite{mccorry2018smart} suggest miners can be bribed to mine empty blocks, effectively performing a \textit{Goldfinger attack}, by receiving an external compensation for devaluing or destroying a cryptocurrency. 
%% not to waste mining power
%Ko{\v{s}}\v{t}{\'a}l  \textit{et. al}~\cite{kovst2018transition} suggest that Bitcoin miners will likely start to mine an empty block as soon they receive a new block. This way they do not waste hashing power while they perform a slow verification of the incoming block transactions simultaneously. When the verification is complete, they know which transactions were included and may go back to mining a new block that does not include them. 
In our work, we observed that 1.43\% of Ethereum blocks are empty and most mining pools mined empty blocks, which suggests mining empty blocks pays off.


==> res_blockchain.tex <==
%%%%%%%   BLOCKCHAIN EFFICIENCY   
\subsection{Blockchain Efficiency}
\label{subsec:blockchainEff}
We now focus on higher level aspects of Ethereum, from the perspective of a blockchain platform.
We focus on aspects that are important to both end users, such as transaction commit time, and miners, such as mining empty blocks.



When an application observes a new block B, it is not safe to immediately consider the state transition given by its transactions, because there is a chance that B might be discarded due to a fork. Thus, applications must wait for a \emph{long enough} suffix of blocks to ensure that the appearance of an alternative heavier chain, not including block B, has a small probability. This property is known as block finality.
Applications choose the probability of chain replacement they are willing to tolerate (i.e., the probability of a block not being final) and wait for enough confirmation blocks to ensure that probability.  
In Ethereum, it is generally accepted that applications should wait for 12 confirmation blocks before considering a block B as final and its transactions as committed~\cite{bez2019scalability, OnAvailability--01, Buterin2015}.
%Note, however, that due to the nature of Proof-of-Work (PoW), block finality is always probabilistic as there is always a non-zero chance that an alternative heavier chain appears.


%We investigate a wide range of blockchain properties with the purpose to identify the behavior traits of both: end users and miners.
%jb: Even if our measurements are similar to Weber's, ours were obtained from multiple observers, therefore we are able to take more meaningful conclusions since we also take geographical location into account.
% DV  :   I  modified the text so it does not sound that bad that we only replicate measurements
% but I comment out the  note about the fact that we are better because we do measurements from more observers while they just from one.  this is because  in this subsection we measure blockchian properties,  not network,   so the fact that we  take geo location into account does not give us any  advantage    In this subsection..
% COMMENTED OUT - While they performed the measurement from one observation point, we used multiple observers     .... enabling us blabla.

% thesis 6.4  tx commit time
\subsubsection{Transaction commit time}
We measured the difference between the time when a transaction was first observed by our measurement nodes to the time at which it was included in a block. 
To determine the block confirmation time, %(\S\ref{bg}), 
we also measured how much additional time it took for such a block to be followed by different numbers of blocks in the main chain. 
These are the metrics that mostly affect end users, and they have a direct impact on user perceived latency.
Figure~\ref{fig:tx-commit-time} shows the times of first inclusion of transactions in a block, and the 3-, 12-, 15-, and 36-confirmation block times.
%jb: the background section only mentions the 12-block case. %(we should explain somewhere why the other variants may make sense for some applications (according to their requirements on the probability that the commit/finality/confirmation properties will hold). maybe in the background section (a simple sentence), and then here briefly remind that again?)
%dv ::  i did the sentence below and i think it's fine
The variants other than the regular 12-blocks case make sense for some applications depending on their requirements regarding block finality probability. % (\S\ref{bg}). 
Besides, as we discuss in \S\ref{subsec:sec}, for applications concerned with the blockchain security, waiting just for 12 blocks might not be enough.
Our measurements revealed that the median waiting time for 12 blocks  was 189 seconds whilst in 2017 it was 200 seconds~\cite{OnAvailability--01}.
The cause for this is that the inter-block time decreased, %\footnote{https://etherscan.io/chart/blocktime} 
from 14.3~seconds to the current 13.3~seconds~\cite{Etherscan2019}.
%To prove that, it suffices to subtract 12 times the mean inter-block time from the time for '12-block commit'. In both cases, we end up with a 29-seconds-long average delay for including a transaction into a block.
This is likely to be related to the Ethereum Constantinople fork that occurred on February 2019 to decrease the inter-block time, which was slowly increasing due to a known hard-coded difficulty bomb \cite{Eips1234, Jameson2019}.

%This exact measurement had been performed in~\cite{OnAvailability--01} where the authors had chosen to measure the commit times for 3, 12 and 36 confirmation. We follow them in order to be able to compare our results with theirs.
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{images/5-3}
	\caption[Transaction Commit Time]{Time for transaction inclusion and commit with 3, 12 (default), 15 and 36 block confirmations.}
	\label{fig:tx-commit-time}
	\vspace{-0.2cm}
\end{figure}



\subsubsection{Transaction reordering}
The transaction creator stamps every transaction with a monotonically increasing nonce. % (\S\ref{bg}). 
We say that two transactions from the same sender were received out of order when we first observe the transaction with the higher nonce. 
Miners cannot include out-of-order transactions in a block until they receive all foregoing transactions, 
which implies that out-of-order receptions negatively impact transaction commit times, as such transactions must wait for their delayed predecessors before committing.
In 2017, 6.18\% out of all committed transactions were received out-of-order~\cite{OnAvailability--01}.
%this was confirmed by a measurement study of Ethereum, where they measured that 
In our measurements, we observed 11.54\% out-of-order committed transactions, a substantial increase.
%suggesting for an increasing occurrence of out-of-order receptions.
% skip.. not needed detail:
%We observe, however, that the proportion of out-of-order transactions fluctuates from day to day between 7\% - 15\% from our one-month average.
We also observed that it takes less than 192 and 325 seconds for 50\% and 90\% of out-of-order transactions to commit.
In comparison, the median time for in-order received transactions is less than 189 seconds and 90\% of these transactions need 292 seconds or less to commit.
The results are depicted in Figure~\ref{fig:tx-reord}.

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{images/5-4-ONE-MONTH}
	\caption[Transaction commit delay based on ordering]{Commit delay (sec) for transaction based on ordering.}
	\label{fig:tx-reord}
	\vspace{-0.2cm}
\end{figure}


%Just like the authors of~\cite{OnAvailability--01}, we do not have a good explanation for the existence of out-of-order received transactions.
%We hypothesize that this might be due to external factors, such as the varying motives of Ethereum users, or the overall network connectivity in the presence of node churn.

\iffalse % begin comment out
%  6.7  gas used per tx type
\subsubsection{Gas used per transaction type}

Ethereum distinguishes between three types of transactions: i) regular value transfers, ii) contract function calls and iii) contract creations.
These are distinguished as follows.
%TODO: mm this should go into the background
A transaction creates a contract if the address of the recipient is empty, as defined in the Ethereum specification~\cite{Yellow}.
%There is, however, no consensus about how to distinguish between regular value transfers and contract function calls.
%In~\cite{OnAvailability--01}, the authors simply say that messages that are not contract creations, and consume 21~GWei of gas (which is the base cost of a transaction), are regular transfers. The remaining messages are function calls.
Transactions that are not contract creations and whose data field is empty are regular transfers.
Finally, transactions with some data (a message for a contract) are contract calls.

% number of each type
Out of 21~960~051 captured transactions, we considered only the subset of 20~654~578 valid transactions included in main blocks.
Of those, there were 8~917~902 regular value transfers, 11~642~182 contract calls and 94~494 contract creations.

\begin{table*}[h]   %[H] / [h]
\centering
	\begin{tabular}{ccccc}
	\toprule
    	{\textbf{Transaction Type}} & {\textbf{\# Transactions}} & {\textbf{Median}} & {\textbf{75th percentile}} & {\textbf{90th percentile}} \\ \midrule
    	{value transfer}  & { 8~917~902}  & {25.2}  & {50}  & {100} \\
    	{function call}  & {11~642~182}  & {100}  & {250}  & {1~000} \\
    	{contract creation}  & {94~494}  & {1~065}  & {1~600}  & {4~000} \\ \bottomrule
	\end{tabular}
\caption[Gas used per Transaction Type]{Gas Used (in GWei) per Transaction Type.}
\label{tab:gasUsed}
	\vspace{-0.4cm}
\end{table*}

As detailed in \S\ref{bg} transactions consume gas.
Table~\ref{tab:gasUsed} and Figure~\ref{fig:tx-gas-used} depict the gas used by each transaction type.
As can be observed, contract creations use the most gas. 
This is because their code consists of computationally expensive routines. 
The median gas used for this type of messages experienced a twofold increase since 2017 to 1~065 Gwei, implying that developers deploy more complex and more computationally expensive contracts. 
Five percent of contract creation messages consume more than 4~500 GWei, which is more than the gas limit per block back in 2017. The current block gas limit is at 8~000~GWei while in 2017 it was only at 4~000~GWei.
This change has done to support more complex Smart Contracts in the Ethereum platform.
The median gas used per function call is 100~GWei and 25.2~Gwei in the case of a regular transfer.
These are relatively small numbers leading to reasonable values of transaction fees.


%Txs TOTAL:  21960051
%Txs TOTAL (after drop):  20654578
%     tot #    min    max       med      aver
%TX: 8917902 21000.0 8000029.0 25200.0 71076.50712308793
%MC: 11642182 21004.0 8007840.0 100000.0 306898.20332468604
%CC: 94494 53000.0 8000028.0 1065269.0 1392285.3344974285
%reg tx  :50%% percentile: 25200.0
%Msg call:50%% percentile: 100000.0
%con crea:50%% percentile: 1065269.0
%reg tx  :90%% percentile: 100000.0
%Msg call:90%% percentile: 1000000.0
%con crea:90%% percentile: 4000000.0
%reg tx  :95%% percentile: 210000.0
%Msg call:95%% percentile: 1000000.0
%con crea:95%% percentile: 4500000.0
%reg tx  :100%% percentile: 8000029.0
%Msg call:100%% percentile: 8007840.0
%con crea:100%% percentile: 8000028.0



\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{images/5-5-txs-gasUsed}
	\caption[Gas Used per Transaction Type]{Distribution of gas usage for different types of transactions.}
	\label{fig:tx-gas-used}
	\vspace{-0.4cm}
\end{figure}

\fi % end comment out



%  dv : we skip this because we haven't confimed the thing below:  
% we also captured 880 suspicious never committing txs that were included in forks - indicating double spending,.... but we havent proved it so we ommit.. and very likely it wasnt double spending attack
%  and never comm. txs alone aren't that    interesting,....   there is not much to say.
%  6.9 never committing txs
%\subsubsection{Never committing transactions}
%There are transactions in the network which will never commit. This is because there already exists another committed transaction with the same nonce which originated from the same account.
%These transactions are useless and flood the network, so we were interested in finding out how many of them there are.

%Out of 21~241~139 uniquely observed valid transactions we find that 20~654~578 (97.2386\%) of them are already committed, 63~446 (0.2987\%)  are not committed but still may commit and 523~115 (2.4627\%) will never commit.

%The transactions labeled as "may commit" are those transactions that had not committed yet, and in addition do not satisfy the condition for being "never-committing".






% empty blocks
\subsubsection{Empty blocks}

We now focus on a set of metrics that affect the behavior of the miners.
Blocks have a maximum number of transactions they can include and currently most blocks are at around 80\% capacity~\cite{Etherscan2019}. %\footnote{https://etherscan.io}.
In principle, miners are incentivized to include transactions in a block because they collect the fees associated with each transaction.
However, miners may occasionally decide to create and propagate blocks that
include no transactions. This behavior grants them the possibility of starting to mine earlier than other miners. 
This has interesting consequences.
On the one hand, miners are penalized by not collecting transaction fees.
On the other hand, they still get the mining reward which is, on average, considerably higher.
Besides, empty blocks can be propagated earlier, because miners do not waste time validating transactions, and faster, since they become smaller due to the absence of transactions. 
Overall, these constitute a perverse incentive to mine empty blocks. As a matter of fact, empty blocks are harmful to the network because they increase the commit time of transactions, as transactions that could have been included in an empty block must wait to be included in the next block. 
If a dominant number of miners switched to the selfish strategy of occasionally mining empty blocks, it would be disastrous for the platform.
To assess the impact of this, we measure the number of empty blocks in the network, and the mining pools from which they originate.
The results reveal that 1.45\% are empty blocks (2,921 out of 201,086 total main blocks). This significant fraction of empty blocks decreases transaction throughput, by increasing the transaction commit delay. 
%If we consider forks caused by empty blocks, we measured 185 forks out of a total of 15~585, which is a slightly lower empty block presence (1.19\%) than in the main chain.

%Therefore, it shows that empty blocks indeed become part of the main chain more often than blocks containing transactions. 
%The second observation is that their number (1,430\% of all blocks) is not insignificant. They are already prolonging the commit times of transactions. (as they don't carry any txs)


Figure~\ref{fig:ptm-3} shows the 15 biggest pools and their share of empty blocks. 
Remarkably, only a small a portion of pools, e.g. Nanopool or Miningpoolhub1, had not mined any empty blocks during our measurement. 
%TODO: mm plot also the total number of observed blocks here
On the other hand, more than 25\% of blocks mined by the Zhizu pool were empty, without a single transaction. 
% 0xF3A71CC1BE5CE833C471E3F25aA391f9cd56E1AA       6             6
% https://etherscan.io/address/0xf3a71cc1be5ce833c471e3f25aa391f9cd56e1aa#mine
% It seems it has mined 128 blocks so far and all of them were empty:
% https://etherscan.io/blocks?m=0xf3a71cc1be5ce833c471e3f25aa391f9cd56e1aa&ps=100&p=2
We also observed a miner whose 6 mined blocks during the experiment were all empty. Etherscan data confirms this miner has systematically only mined empty blocks since its account was created~\cite{Etherscan2019}.

We can therefore conclude that the mining of empty blocks varies substantially across mining pools, which shows that this practice depends on the specific protocols and policies used by each mining pool.
The fact that one major mining pool resorts to this practice frequently might show that the benefits of this selfish behavior are relevant.
This, in turn, may suggest that this behavior may be replicated more aggressively by other mining pools in the future, which will imply higher penalties on the commit delay.
%While empty blocks are a safety mechanism that allows the network to make progress under certain situations, for instance during an upgrade of the Ethereum protocol, it is clear that additional measures are needed to prevent a wide adoption of this practice. 

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{images/ptm-3-empty-blcks-per-miner.pdf} 
	\caption[Block Commit Time]{Empty blocks per mining pool.}
	\label{fig:ptm-3}
	\vspace{-0.6cm}
\end{figure}





\subsubsection{Blockchain forks}
\label{subsubsec:forks}





In our measurement, we were able to observe nearly all blocks that were created on the network.
This included 485 unrecognized forks that are not reported by popular Ethereum blockchain explorers like Etherscan~\cite{Etherscan2019} or Etherchain~\cite{Etherchain2019}. %\footnote{etherchain.org}.
%This sentence is not about results, it is mostly about showing that our methodology was accurate.

%Then, we performed a complementary measurement on single peer with default settings from May 2nd to May 9th, for the needs of metric in Section~\ref{section:reception_redundancy}.

%Main: 201086 rate: 0.9280706693558437
%Unrec Uncle: 485 rate: 0.002238416770126136
%Recognized Uncle: 15100 rate: 0.06969091387403022

%e we distinguish between forks of lengths one, two and possibly longer ones. We also calculate the proportion of observed forked blocks and the total number of blocks.

Out of the 216,671 blocks that we captured, 92.81\% of them became part of the main chain, 6.97\% became uncles referenced by some block from the main chain and only 0.22\% of the blocks became unrecognized uncles. 
Table~\ref{tab:forkedblocks} also shows that forks of length one are the most common (97\%) and that the longest forks observed were of length 3. It also shows that forks of length one are very likely to become recognized, i.e. referenced as uncle in some main block. During our measurement, not a single fork longer than 1 became recognized.

\begin{table}[h]   %[H] exact pos [h] aprox [t] top [b] bott - [ht] combinations..
\centering
	\begin{tabular}{ccccccc}
	\toprule
    	{\textbf{Fork Length}} & {\textbf{Total}} & {\textbf{Recognized}} & {\textbf{Unrecognized}} \\ \midrule
    	{1}  & {15,171}  & 15,100  & 71   \\
    	{2}  & {404}  & 0  & 404   \\
    	{3}  & {10}  & 0  & 10    \\ \bottomrule
	\end{tabular}
\caption[Fork Lengths]{Fork types and lengths.}
\label{tab:forkedblocks}
	\vspace{-0.4cm}
\end{table}




Since 2017, the proportion of forked blocks increased by more than one percent and their lengths increased as well.
Among other possible factors, it is likely that this trend reflects the fact that mean inter-block time (the time between two succeeding blocks) has decreased
by around one second in the last two years~\cite{Etherscan2019}.











%ptm-6    gd5(+4)
\subsubsection{One-miner Forks}
The Ethereum yellow paper defines fork as ``a disagreement between nodes as to which root-to-leaf path down the block tree is the best blockchain''~\cite{Yellow}.
Forks are thus expected to occur when distinct miners disagree on the best blockchain (e.g., on distinct versions of the highest block produced by distinct miners), but not due to a single miner producing distinct blockchains simultaneously (e.g., distinct versions of the highest block).
Surprisingly, we find many instances where a single miner produced several blocks at the same height.
%However, we find that many miners produce blocks with the same height, thus creating disagreements not just between different miners but also inside individual peers.
This phenomena, which clearly was not foreseen in the original specification, has a relevant impact today.
In fact, more than 11\% of all forks consisted of a divergence between two blocks from the same miner.

We find that miners produced 1,750 block pairs with a unique block height. They also mined 25 triples of blocks, once mined a 4-tuple and once a 7-tuple of such blocks.
In the case of the 4- and 7-tuples, we believe that these were due to a mining pool partition or another pool malfunction.
In the case of a 3- and 2-tuples, there is a strong reason to suspect of intentional behavior: these forks got recognized as uncle blocks and thus got rewarded in 98\% of the cases.
This phenomenon shows that the uncle block rewarding system, which was intentionally meant to help less powerful miners, is effectively helping the most powerful mining pools to unethically profit from multiple rewards, by mining multiple versions of the highest block in parallel.




%To summarize, in this section, we replicate several measurements on Ethereum blockchain properties done by Weber \textit{et. al}~\cite{OnAvailability--01} in 2017 enabling us to compare how the platform evolved since then. 
%We show that Ethereum, in just 2 years, experienced an increased number of forks by one percent, an increase in the time needed for transactions to commit, and an increase on the average complexity of deployed Smart Contracts.
%Interestingly, we also found that some miners are exploiting the uncle reward system in unexpected ways as well as the mechanism that allows the mining of empty blocks.


==> res_geoimpact.tex <==
\subsection{Geographical Impact}
\label{subsec:geoImpact}
%jb:
%maybe it would be good if, at each section (4.1, 4.2, ...) we included:%- a paragraph with some initial context about the focus of this section (for instance, referring to the contents of the bground section to explain why this section is important, etc).%- we should say what are the main questions that we want to answer on this section (this helps the reader proceed to the details of the analysis, since he expects a priori the main things we want to determine)%- a short itemize (3-5 items) summarizing the most important findings (short items)
%The Ethereum network works by disseminating transactions and blocks among the set of peers, as detailed in \S\ref{background}.
%If the network is slow in disseminating transactions this means that end users will observe a large latency in the transactions they submit to the system.
%Regarding blocks, a slow block propagation has harsher consequences, since this will lead to more forks as miners are not aware of each other's blocks in time.
%It is therefore crucial to have low propagation delay for both transactions and blocks.

We now study the impact that geographic location has on block propagation delays. 
This is important because, if some region has lower propagation delays than others, that region has an advantage when mining new blocks, as miners will become aware of the latest blocks faster and thus can start mining the next block ahead of miners in other regions.
%As discussed above, the propagation delay of transactions is very small and in the order of our measurement error and therefore we do not further study transaction propagation delays.

%Good interconnection of peers and fast propagation times of transactions and blocks are crucial for Ethereum to keep the platform synchronized.
%   why blocks and not txs
%  dv thesis:The median time until a node receives a transaction is just 60 mili-seconds
% NTP over the Internetin 99 % of cases offsets <100 ms;  90 % <10 ms
 
%The final reason why our measurements focus on block messages rather than on transactions is that blocks play the prime role in platform synchronization and their faster observation gives a great advantage for miners by providing them an extra time to spend on mining.

% itemize 3-5   findings..

%Regarding transaction propagation delays, we did not find them to be affected by geographic location.
%The two main factors that explain this: i) transactions are small and propagate faster (within the NTP precision range); ii) transactions tend to be created in a more geographically dispersed fashion (transactions are submitted from a large set of nodes) as opposed to blocks (where just a few miners are produce most of them).
%
%
%Our measurements revealed that: (i) 99\% of blocks propagate under 0.317~ms, (ii) the geographical placement of nodes indeed affects propagation times, (iii) majority of blocks are to be seen in Western Asia first. 

%###### blocks
%median 0.07400000000000001
%average 0.10902917934723612
%:50%% percentile: 0.07400000000000001
%:90%% percentile: 0.171
%:95%% percentile: 0.21100000000000002
%:98%% percentile: 0.267
%:99%% percentile: 0.317
%:100%% percentile: 673.7230000000001




%PTM-4-A   G1, G2
%GEO. POSITION of nodes VS block rec. times (e.g. Taiwan first)
\subsubsection{Geographical position influence}
\label{subsec:geo-influence}

The Ethereum network establishes neighboring relationships among peers based on a random node identifier. 
This is independent of the geographic location and therefore, assuming that the network capacity (bandwidth and latency) is evenly distributed among miners, nodes should observe similar propagation delays regardless of their location.
Regarding transaction propagation delays, we did not find evidence that
they were affected by geographic location (results not shown for space limitations). However, we found that block propagation delay is affected by geographic location.
%There are two main factors that explain this observation: i) transactions are small and propagate faster than blocks and within the margin of our measurement error (\S\ref{bg}), and  ii) transactions tend to be created in a more geographically dispersed fashion (transactions are submitted from a large set of nodes) as opposed to blocks (where just a few miners are produce most of them).


%lghboring y forms a random graph as the peer selection is determined by random node ID lookups, independent of geographic location.
%If this claim holds in practice, every node should measure similar average propagation delays.
To assess this, we measured the proportion of times each of our measurement nodes was the first to observe a new block. 
%, reg that ended up utime difference between new blocks across the different geographical locations.
The results are depicted in Figure~\ref{fig:geo-position-vs-block-observ-time}.
%We wanted to verify that claim by comparing the new block observation times between peers placed on different geolocations.
%not easy to read this sentence.%why 10ms?%"NTP block synchronization" is confusing, since the reader may question "is NTP related to block synchronization???"%Please revise (or even sub-divide into 2 sentences) to clarify.
% shows, for each of our measurement nodes, the proportion of first new block observations.
%mention error bars?   I skip it as it is in the title...
%%%%% jb:
%why is this? can we say something about possible factors?%isn't this result already studied by others? if so, we should acknowledge and compare our results with those older ones.
The results clearly show that nodes located in EA are the first to receive new blocks most of times ($\approx$40\% of times) whereas nodes in North America are around four times less likely to observe  new blocks first.
Therefore, the geographical location of nodes affects the new block observation times and therefore miners in EA are at an advantage.
The cause of this, as we show in the following measurement, is simply due to the fact that several prominent mining pools operate in Asia and therefore nodes in EA are more likely to receive new blocks first. %It is, however, needed to remind the reader that the overall block propagation delays are low -- in 99\% of times they are below 317~ms.

%We note that the geographical concentration of large mining pools does not have
%a similar effect on transaction propagation delays. In contrast to blocks, 
%which are mostly disseminated from a small subset of nodes (the gateway nodes of mining pools), transactions tend to be created in a more geographically dispersed fashion (transactions are submitted from a large set of individual nodes).



\begin{figure}[t]
 \centering
 \includegraphics[width=\linewidth]{images/ptm-4-geo-position-vs-block-observ.pdf}
 \caption[Block propagation]{First new blocks observations with respect to geographical location. The error bars represent the experimental error (\S\ref{methodology}).}
\label{fig:geo-position-vs-block-observ-time}
	\vspace{-0.2cm}
\end{figure}

%ptm-4-c  G2
\subsubsection{Mining pools' location}


The emergence of huge mining pools does not only centralize mining power on a few entities, it also centralizes (on a few geographical hot-spots) block propagation. 
To overcome this, and counter the effect observed in the first experiment, mining pools have been known to place gateways in several geographical locations in order to help disseminate their blocks, without disclosing their precise location to avoid attacks \cite{miller2015discovering}. 
To study the impact of this, we measure whether our geographically dispersed measurement nodes capture blocks mined from particular mining pools faster than from others.
The results are depicted in 
%In order to confirm our assumption, that the gateway(s) of each mining pool are not geographically centralized -- i.e., not uniformly spread across the globe -- we extended the previous metric and measured whether our geographically dispersed instances capture blocks mined from particular mining pools faster than from others.
Figure~\ref{fig:ptm-4-c}, which shows first new block reception per individual mining pool. 
We consider only the 15 most prominent mining pools, since the fractions of blocks produced by the smaller pools are insignificant. %Figure~\ref{fig:pool-distr}.
The results clearly show that the geographic location of peers affects faster block observation from certain pools, and indicates that the gateways of mining pools are not evenly distributed.
 
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{images/4-c-miners-vs-our-instances-10msPrecis.pdf} 
	\caption[Block Commit Time]{The influence of a block's origin mining pool on the faster propagation times to various geographical locations. 
	In parentheses, we show the computational power of each mining pool during our experiment.} %Top 15 mining pools ordered by computational power.}
	\label{fig:ptm-4-c}
	\vspace{-0.2cm}
\end{figure}


%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{images/eth-top-miners}
%	\caption[Distribution of Ethereum mining pools]{Mining pools' capacity distribution from April 18th 2019 to April 25th 2019 (etherscan.io).}
%	\label{fig:pool-distr}
%	\vspace{-0.2cm}
%\end{figure}  %\footnote{https://etherscan.io/stat/miner?blocktype=blocks}


%To summarize, these measurements show that the geographical location of nodes indeed affects block propagation times, with majority of blocks being observed in EA first. 
%Therefore, a miner that wishes to maximize their potential gains should place her computing resources in that region.


==> res_neteff.tex <==
\subsection{Network Efficiency}
\label{subsec:netEff}
%- a paragraph with some initial context about the focus of this section (for instance, referring to the contents of the bground section to explain why this section is important, etc).%- we should say what are the main questions that we want to answer on this section (this helps the reader proceed to the details of the analysis, since he expects a priori the main things we want to determine)The information in the Ethereum network propagate fairly fast, as Section~\ref{subsec:geoImpact} shows.

The Ethereum network disseminates transactions and blocks using a gossip-based protocol. %, as detailed in \S\ref{bg}.
If the network is slow in disseminating transactions this means that end users will observe a large latency in the transactions they submit to the system.
Regarding blocks, a slow block propagation has harsher consequences, since it will lead to more forks as miners are not aware of each other's blocks in time.
%It is therefore crucial to have low propagation delay for both transactions and blocks.
Therefore, this section studies the efficiency of Ethereum's network, focusing
on the propagation of blocks.
More precisely, our focus is on understanding how fast the Ethereum network
propagates blocks and on whether it generates significant message redundancy.
%, as well as how network-efficient it is in doing that reliably.% it makes use of the network resources.

% At the same time, propagation should be redundant enough to ensure that transactions and blocks reach every node reliably. Yet, this redundancy should be optimized to not overload the limited capacity of the network.

% In order to get a better picture of the network's condition, we analyzed
% transaction and block propagation messages received at each measurement node
% of our platform.

%with the intent of understanding the 
%Our analysis focu all the traffic and particularly were looking for propagated information that is useless, or for the actual number of redundant blocks received by individual peers.

%- a short itemize (3-5 items) summarizing the most important findings (short items)
% We found that: (i) the prevalent block propagation method is direct rather than via announcements, (ii) the amount of redundant block messages is close to optimal. (iii) We capture the presence of peers from competing platforms causing significant and undesired noise.


%PROPAG. DELAYS
\subsubsection{Block and Transaction Propagation Delays}
\label{subsec:block-propag-times}

% We start by describing our methodology to measure propagation delays.
% One naive approach would be to compare the time at which transactions/blocks are received at a measurement node with the timestamp that each transaction/block carries, which are set by the node that generated the transaction/block -- respectively, the transaction sender or the block miner.
% However, this timestamp is unreliable, not only because it can be freely set by the latter node, but also because we cannot make assumptions about the synchronization of those nodes' clocks.

% Therefore, we adapt the method proposed by Decker et al. \cite{InfPropagaion--02}, which exclusively relies on timestamps generated by our measurement nodes to compute the block propagation delay. More precisely, we define propagation delay (of a transaction or block) as the time difference between the first observation of a block at any instance of a measurement node and the times of arrival on the remaining measurement nodes. 

% Note that this is an approximated method since (i) it does not measure the time it takes to propagate a
% transaction or block from the source node (transaction sender or block miner)
% to the first measurement node that received that transaction or block; and (ii) the accuracy of our measurements is always bounded by the accuracy of NTP in synchronizing the local clocks of our measurement nodes.
% This this level of accuracy is not acceptable for transactions, which are short and typically propagate at a low latency. Still, this method is sufficiently accurate to characterize the (longer) propagation delay of blocks.

%Therefore, this section focuses on block propagation delays.


%but rather the relation between geographical location and propagation delays.

%This is could happen if all our monitoring nodes were far from the miner.
%jb: why calculating delay using the TS on the block is not meaningful.
%Block messages only contain a timestamp which is lacking precision as it is freely set by miners.
%Therefore, we rather rely on our own infrastructure's timestamps. Like~\cite{InfPropagaion--02}, 
%we define the propagation delay of a block as the difference between its first observation at any instance from our measurement infrastructure and the times of arrival on the remaining nodes. 
%For instance, if a block is observed by our four instances for the first time at times: 20, 10, 12, and 15; the the delays are: 10, N/A, 2 and 5. 
%jb:it would be cool to elaborate why this definition makes sense. 
%   and   why it is fair to say that the first node to receive a block observed zero delay. (Because, in reality, there is always some propagation delay, even to the first observer node to receive the block.)
%The weak spot of this measurement strategy is that it does not precisely measure the exact time it takes to propagate a block from a miner to nodes This is could happen if all our monitoring nodes were far from the miner.
%We were, however, more interested in observing the correlation between the geographical distance of nodes and the propagation delays, which this method captures precisely.





\begin{figure}[t]
	\centering
	%\includegraphics[width=\linewidth]{images/5-1-png-exported} % PNG only to save some mem
	%\includegraphics[width=\linewidth]{images/5-1-block-propagation-times} %BEST QUALITY but 5MB
	\includegraphics[width=\linewidth]{images/5-1-OLD-buckets} % OLD   w/ buckets
	\caption[Block propagation times]{The histogram of times since the first block announcement.}
	\label{fig:information-propagation}
	\vspace{-0.2cm}
\end{figure}


Figure~\ref{fig:information-propagation} depicts the results for block propagation delays.
The median block propagation delay was 74ms and the average was 109ms. 
The propagation delay of the 95\% fastest blocks was under 211ms, and it took 317ms for 99\% of blocks to propagate through the network.
This shows that blocks are propagated several orders of magnitude below the
average inter-block time (currently 13.3s). 
%Hence, block propagation delay is unlikely to be a relevant cause of forks.


Regarding transaction propagation delays, we did not find them to be affected by geographic location (results not shown due to space constraints).
There are two main factors that explain this observation: i) transactions are small and propagate faster than blocks and within the margin of our measurement error (\S\ref{methodology}), and  ii) transactions tend to be created in a more geographically dispersed fashion (transactions are submitted from a large set of nodes) as opposed to blocks (where just a few miners produce most of them).

%and slow block propagations are not the main cause of forks as pointed out in previous studies in the Bitcoin network~\cite{InfPropagaion--02}.



% %(PTM-2): Forks-observed-before-main-blocks
% %15 585 forked blocks (uncles+unrecognized) we captured 3 928 forks
% To further confirm this, we measured the time difference between observing blocks at the same height, and hence leading to forks.
% We found out that despite observing first a block B and later a block B' at the same height, $\approx$25\% of the times (3~928 out of 15~585 ) block B' ended up in the main chain and block B' as an uncle.
% This indicates that miners continued mining blocks even after discovering competing blocks of the same height. 
% They can afford that due to the uncle rewards, which are almost guaranteed for forks of length one, as we discuss in more detail in \S\ref{subsubsec:forks}.

%happen and found out that 3~928 out of 15~585 ($\approx$25\%)<++>forked blocks, in spite of being observed before their corresponding main block, they did not end up in the main chain.  

%I'm afraid the reviewer will not understand how "avg latency between nodes" relates to "block propagation delay", and he'll get lost here... %You define the latter, but not the former.%If each term is defined differently, you should clarify the definition of "latency between nodes" and how it related to "block prop. time".%If both terms mean the same thing, you should consistently use the same term to avoid misunderstandings.

%\jpb{I have problems with the paragraph below: (i) it is not clear how this ``average latency between peers'' relates to our metric of block propagation delay, which is really confusing for the reader; (ii) we don't have a proper explanation for the difference in values (the possible explanations are too vague and speculative, making this observation meaningless). I suggest we remove this paragraph.}
%%smoothed round-trip times measured on direct connections, which
%Kim \textit{et. al}~\cite{MeasEthPeers} in 2018 measured the average latency between peers based on smoothed round-trip times measured on direct connections to be at 173~ms. We measured more than 90\% of blocks to propagate even faster than that. This indicates that either our instances were connected directly to the gateways of major mining pools or that there are some highly connected peers helping block propagation.
%This would not be surprising since mining pools are encouraged to disseminate blocks as fast as possible in order to increase the chances of their blocks becoming part of main chain.


\subsubsection{Block reception redundancy}
Blocks are disseminated through two types of messages: either in the form of light announcements (consisting of only the block's hash) or propagated directly (including both header and body).
The dissemination protocol has builtin redundancy mechanisms to tolerate faults and packet loss. % (\S\ref{bg}).
However, such redundancy comes at the cost of additional network delays and processing overhead.
Therefore, we are interested in knowing how many redundant blocks a node with default settings receives.
Because our measurement nodes are connected to more nodes than the default (\S\ref{methodology}), we performed a subsidiary measurement for this metric, between May 2\textsuperscript{nd} 2019 and May 9\textsuperscript{th} 2019, where an additional measurement node was connected to the default number of peers (25).
\begin{table}[t]
\centering
	\begin{tabular}{ccccccc}
	\toprule
    	{\textbf{Message Type}} & {\textbf{Avg.}} & {\textbf{Med.}} & {\textbf{Top 10\%}} & {\textbf{Top 1\%}} \\ \midrule
    	{Announcements}  & 2.585  & 2 & 5 & 7  \\
    	{Whole Blocks}  & 7.043  & 7 & 10 & 12  \\
    	{Both combined}  & 9.11  & 9 & 12 & 15   \\ \bottomrule
	\end{tabular}
\caption[Redundant Block Receptions]{Redundant block receptions.}
\label{tab:redundantblockreceptions}
	\vspace{-0.2cm}
\end{table}
%this seems a weak support for our conclusion (some work *suggests*...).%we should cite works that *prove* this, rather suggesting this.
The results are depicted in Table~\ref{tab:redundantblockreceptions}, which shows that blocks are more often propagated directly rather than via announcements.
The median and mean number of redundant block message receptions is 9.00 and 9.11, respectively, considering both announcements and direct block propagation messages. Even the top~1\% of most redundantly propagated blocks are received just 15 times. 
Eugester et al.~\cite{EpidemicDistr} show that, in networks with failures, it is enough for the gossip protocol to disseminate information to a logarithmic number of neighbors with respect to the total system size.
According to the latest estimation from~\cite{MeasEthPeers}, there are around 15,000 Ethereum peers.
Therefore the measured mean of 9.11 block receptions is close to the optimal value of 10 ($\ln(15,000)$ $\approx$ 9.62).
This is further confirmed by the low propagation times analyzed in \S\ref{subsec:geoImpact}.

\iffalse % begin comment out
\subsubsection{Ethereum classic traffic}
Every message -- such as block announcement, connection attempt or new transaction -- received by an Ethereum client must pass through a validation phase before it is processed. One important validation is the DAO check~\cite{AttacksSurvey}.
We captured all these failed verifications and observed between 10~388 to 24~798 -- depending on the measurement instance -- of block header messages that failed due to the DAO check.
Therefore, we confirmed the presence of Ethereum Classic peers, i.e. an alternative blockchain that considers the blocks involved in the DAO attack~\cite{AttacksSurvey}.
This is undesirable because such nodes run an alternative blockchain and hence flood the network with useless information.
The reason for this is because Ethereum operates on a DEVp2p network, which is shared with other platforms as well. Most current Ethereum's client implementations do not prohibit connecting to peers from incompatible platforms, resulting in useless traffic.
This observation confirms the prior findings of Kim \textit{et. al}~\cite{MeasEthPeers}.
\fi % end comment out

% DV  :   I skip this (even though it is true what is there)
%         because  it does not relate to ETC traffic and we already have 13+ pages..
%On top of the Ethereum classic traffic, we captured just 17 invalid network messages, all of them were of one type - decoding error of transaction message. That is an insignificant number in comparison with billions of transaction messages, thus we have not observed any significant noise of useless traffic flooding the network.

% Only after finishing our measurements a new version of Geth - 1.9.0\footnote{https://blog.ethereum.org/2019/07/10/geth-v1-9-0/} was released which implements Ethereum Node Record (ENR) extension of the discovery protocol. It allows to filter out unwanted connections including the problematic Ethereum classic ones. It will, however, take some time until all participants update to the newest Geth version and the other client implementations switch to ENR as well.


==> res_sec.tex <==
\subsection{Security} % censorship
\label{subsec:sec}

\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{images/ptm-1-cdf.pdf}
	\caption[Block Commit Time]{The sequences of consecutive main blocks mined by a unique miner.}
	\label{fig:ptm-1-a}
	\vspace{-0.4cm}
\end{figure}


%- a paragraph with some initial context about the focus of this section (for instance, referring to the contents of the bground section to explain why this section is important, etc).
As previously discussed, mining in Ethereum is performed by a few mining pools that dominate the platform. 
Moreover, miners are free to select which transactions to include in a block and which to discard.
This raises concerns over the security and fairness of the network, as a mining pool might censor transactions from a given user, or perform other attacks such as a double-spend by reverting a suffix of the blockchain.


%Recall that in Ethereum a block B is considered final after B has 12 blocks after it in the blockchain (\S\ref{bg}).
In Ethereum, a block B is usually considered final when it is followed by a 12 block sequence.
If a mining pool is able to produce more than 12 blocks in row, this means that it can effectively censor the blockchain and perform attacks such as double-spends.
A less severe attack that mining pools can perform is to increase the latency of a given transaction simply by refusing to include it in the sequence of blocks they mine.
This %, along with the mining design decision that allows miners to filter transactions, 
enables them to perform a temporary censorship.
%- we should say what are the main questions that we want to answer on this section (this helps the reader proceed to the details of the analysis, since he expects a priori the main things we want to determine)
%Next, we investigate this problem and show to what degree this threat is possible.
To assess the security of the network, from the perspective of block finality, we measured the length of consecutive sequences of blocks created by the same mining pool.
We were interested in the probability of temporary censorship taking place and for how long mining pools would be able to do it.
Our results reveal that Ethereum pools regularly have the opportunity to temporarily censor transactions for more than two minutes, but historically we registered events allowing for 3-minute-long censoring.

%- a short itemize (3-5 items) summarizing the most important findings (short items)

% Mining pools can choose which transactions to insert in blocks, which causes a threat to the Ethereum platform as it enables them to temporarily censor them, thus considerably prolonging their commit times. In the case of the 9-block sequence, the transaction commit could be delayed by almost two minutes.


%describe   FIGURE  our measurement
During our one-month measurement, we observed that the prominent pools managed to mine sequences of blocks as long as 9. 
The results are shown in Figure~\ref{fig:ptm-1-a} which depicts the lengths of consecutive blocks the top 5 mining pools were able to produce. 
Ethermine %, the mining pool with the most capacity (Figure~\ref{fig:pool-distr}) 
managed to mine four 8-block long sequences and Sparkpool was able to generate 9-block long sequences twice. 

%  WHY  dangerous -- they can CENSORE..


%etherime ... ethscan 0.259 ...   probabl   0.259  MATCHES.. exactly
%Ethermine (0.259 out of the total mining power of Ethereum)
%P(seq_8): 0.259^8    =     0.00002  chance     (they managed to do this 4x)

%Sparkpool (0.227 out of the total mining power of Ethereum)
%P(seq_8): 0.227  ^ 8  =     0.000007  	(they managed 1x)
%P(seq_9): 0.227  ^ 9  =     0.0000016    	(they managed 2x)


%There were 201 086 of main blocks.

%The probabilities are not “that” small and there are many new blocks each minute:
% 0.00002 *  201 086 = 4 …   which is exactly the number how many times it happened.
%The biggest pools simply are too powerful so these very long sequences are likely to happen.
%All our previous metrics also did not indicate block witholding.  
%These are caused by the great computational power share that the pools have. According to the blockchain explorer Etherscan~\footnote{https://etherscan.io} the Ethermine's share during our experiment was about 0.259 of the total power. Thus the probability of a nine-block sequences is $0.227  9$ 

At the time of our measurements, the accumulated computational power of all Ethermine's miners was 25.9\% of the whole Ethereum platform~\cite{Etherscan2019}. Therefore, the theoretical chance of mining a sequence of 8 consecutive blocks would be $0.259^8 = $ %2 \times 10^{-5} %  2\mathrm{e}{-10}$ 
$2 \times 10^{-5}$.
During one month, there were 201,086 blocks in the main chain.
With a theoretical chance of $2 \times 10^{-5}$, this means that Ethermine should be able to mine 8 consecutive blocks 4 times per month ($2 \times 10^{-5} \times 201,086 \approx 4$) exactly the value we observed.
In the case of Sparkpool, which has a theoretical chance of mining 9 consecutive blocks of $0.226^9$ it should take at least three months to mine such a sequence ($0.226^9 \times 201,086 \approx 0.3$) however it did so twice in a month.
Since blocks were not announced all together, like in a block withholding attack, and presented an average inter-block time, it is unlikely that Sparkpool performed such an attack~\cite{kwon2017selfish}. It is more likely that the current values that are used to consider a block as final are too optimistic, given the fraction of mining power that is currently held by mining pools.
To further justify this observation, we looked beyond our one-month experiment, and analyzed the whole blockchain.
We observed 102, 41, 4 and 1 sequences of 10, 11, 12 and 14 consecutive blocks, respectively.
The longest sequence ever recorded, consisting of 14 blocks, was mined by Ethermine from block height 5,899,411 to 5,899,424.
We do not know the exact computational power of Ethermine at the time, but if we assume that it was similar to its current power (0.259) the probability of such a long sequence would be around once in 1,000 years.


%LONGEST EVER
%seq-len: 12	pool: DwarfPool1	block nums: 1005215 - 1005226
%seq-len: 12	pool: DwarfPool1	block nums: 1041376 - 1041387
%seq-len: 12	pool: DwarfPool1	block nums: 1252178 - 1252189
%seq-len: 12	pool: DwarfPool1	block nums: 1410893 - 1410904
%seq-len: 14	pool: Ethermine	block nums: 5899411 - 5899424

%Btw, the theoretical chance that a pool with 25.9% computational power of the network would mine 14 blocks in a row without cheating is once in 1 000 years.  
%calculated as follows: (0.259 ^ 14) *  201086 
%where “201086” is the number of blocks mined in one year.
%BUT WE DONT KNOW HOW POWERFUL was   that  mining pool back then..

%This minuscule probability makes us suspicious whether the

%To conclude, these long one-miner main-block sequences represent one of the many dangerous consequences of the current mining power being distributed among such few prominent mining pools.
%Honest miners should switch from the most prominent mining pools to smaller ones in order to prevent this from happening.  
%However, and as we discussed in \S\ref{subsec:blockchainEff}, the current mechanism to incentivize individual or small mining pools are being exploited by mining pools, further reducing the incentive of to small miners.

%ptm 1 a



==> results.tex <==
%%%%%%%%%%%   ANALYSIS   %%%%%%%%%%%
\section{Results}
\label{Analysis}

In this section, we present our measurements and discuss the obtained results in face of our expectations and also, whenever appropriate, how they relate to other studies.
During our one-month measurements, we collected data about 216,656 blocks (including forks) with the block numbers ranging from 7,479,573 to 7,680,658.
On top of that, we captured 21,960,051 unique transactions out of which 20,654,578 (94\%) were valid transactions included in main blocks.

Our study focuses on answering a wide set of questions that depend on distinct, yet cross-dependent, facets of the whole Ethereum platform.
We %do this by 
follow a bottom-up structure.

\iffalse % begin comment out
First, \S\ref{subsec:netEff} characterizes the efficiency of
the Ethereum network as a dissemination protocol whose main purpose is to
disseminate transactions and blocks across the whole system.
\S\ref{subsec:geoImpact} complements the previous results by
studying the behaviour of the network from
a higher perspective that consider the impact of geographic location.
Abstracting one more level, \S\ref{subsec:blockchainEff} focuses
on the efficiency of the blockchain abstraction that is built on top of
such transaction and block propagation network.
At this level, we are interested in understanding how efficiently
(and correctly) transactions reach blocks and, in turn, how efficiently
the main blockchain progresses in incorporating new blocks.
Finally, at the highest level, \S\ref{subsec:sec} investigates
how strongly Ethereum is effectively guaranteeing the (probabilistic) property of block finality.
\fi % end comment out

% The rest of the section is organized as follows: 
% \begin{itemize}
%   \item \S\ref{subsec:geoImpact} discusses the impact of geolocation of Ethereum peers on information propagation times.
%   \item \S\ref{subsec:netEff} studies the efficiency of the Ethereum network.
%   \item \S\ref{subsec:blockchainEff} deals with the blockchain properties.
%   \item \S\ref{subsec:sec} investigates the security aspects of Ethereum.
% \end{itemize}


 \input{res_neteff}
 \input{res_geoimpact}
 \input{res_blockchain}
 \input{res_sec}

